Simulating Parametric Thin Shells by Bicubic Hermite Elements

In this study, we present the bicubic Hermite element method (BHEM), a new computational framework devised for the elastodynamic simulation of parametric thin-shell structures. The BHEM is constructed based on parametric quadrilateral Hermite patches, which serve as a unified representation for shell geometry, simulation, collision avoidance, as well as rendering. Compared with the commonly utilized linear FEM, the BHEM offers higher-order solution spaces, enabling the capture of more intricate and smoother geometries while employing significantly fewer finite elements. In comparison to other high-order methods, the BHEM achieves conforming $\mathcal{C}^1$ continuity for Kirchhoff-Love (KL) shells with minimal complexity. Furthermore, by leveraging the subdivision and convex hull properties of Hermite patches, we develop an efficient algorithm for ray-patch intersections, facilitating collision handling in simulations and ray tracing in rendering. This eliminates the need for laborious remodeling of the pre-existing parametric surface as the conventional approaches do. We substantiate our claims with comprehensive experiments, which demonstrate the high accuracy and versatility of the proposed method.

==> Sections-old/Conclusions-and-Discussions.tex <==
\section{Conclusions and Discussions}

%implementation limitation: contact(IPC, patch self-collision), performance, residual sensitivity, topology change
%Future work: learning and inverse application, IPC, solve PDE on manifold, plasticity, adaptivity

In this study, we propose a new computational framework for direct elastodynamic simulation of parametric thin-shell structures. 
The central piece of our framework is a high order finite element formulation based on bicubic Hermite interpolation. Since the Hermite polynomial shape function ensures $\mathcal{C}^1$ continuity, our interpolation of the $4$th-order KL model promises little numerical simplification, consequently, circumvents the numeric locking issue challenging most of the linear finite element method. 
Capitalizing on the advances in parametric surface modeling and rendering, we develop a continuous collision detection scheme specifically tailored for bicubic Hermite surface. Such a unified approach allows us to achieve high fidelity simulation without resorting to any form of auxiliary tessellation mesh. 
%our method can discretize the continuum KL model without any numerical simplification. This rigorous derivation allows our method can provide higher accuracy and suffer from many numerical issues existed in traditional FEM. 
%High-order methods have some obvious advantages (better convergence behavior in the thin limit, continuous surface normals) at the cost of additional computation and complexity, especially when handling contact
Compared with the state-of-the-arts in IGA, our proposed simulation framework represents a tight coupling between CAD and FEA, which inherently improves performance on fidelity, efficiency, and ease of control.

%implementation limitation: performance, residual sensitivity, topology change

%Moreover, since the present elements involve higher-order derivatives into the nodal degree of freedoms and strictly pass through ,
While our method can efficiently simulate parametric thin shells with better convergence behavior, there are a number of notable limitations. The Hermite interpolation possesses global smoothness, which is more suited for describing characteristic artifacts such as wrinkles or folds of cloth motion. However, plastic deformation and impact dynamics remain a challenging problem due to their nonlinear and non-smooth nature of the response. 
When solving the equation of motion with Newton's method, the unit difference between displacement and its high order derivative is not accounted for. We believe better convergence may be achieved by taking the descent direction with this difference into consideration. 
Our current implementation still can not handle challenging contact scenarios such as tying ribbons into a reef knot. We think that integrating with IPC would make a natural follow-up work, aided by all the major components (continuous/discrete collision detection algorithm )  already established in this work. 
A highly valuable extension of the current framework would be to handle topology changes caused by cutting or tearing.  
Another exciting avenue for future research is extending our fully differentiable formulation to geometric deep learning.

%since the Hermite interpolation precisely
%passes through the sampled function values and maintains their
%first-order derivatives, our method  enables intuitive constraint editing.

%Future work: learning and inverse application, IPC, solve PDE on manifold, plasticity, adaptivity
%which is called Bicubic Hermite Element Method (BHEM). 
%In our method, the quadrilateral patch equipped with Hermite interpolation is utilized as a unified representation for both shell geometry modelling and the computational unit in the finite element analysis. Compared with the commonly adopted linear triangular element, the present Bicubic Hermite elements possess higher-order solution space and higher inter-element continuity in the displacement field (C1 continuity) through involving higher-order derivatives into the nodal degree of freedoms. Thereby, the BHEM can naturally capture smoother and richer geometries with much fewer finite elements, and simultaneously avoid the severe locking troubles known as transverse shear and membrane locking.
%To better facility the seamless integration of the parametric surface representation and the physics-based animation of thin shell, we further developed an efficient Hermite surface intersection algorithm. With this technique, no cumbersome remodeling of the already generated parametric surface model is required any more for the purposed of collision detection and ray-tracing rendering. 
 


==> Sections-old/Implementation.tex <==
\section{Implementation}



\begin{comment}
\subsection{Pipeline}
Our pipeline to simulate each time step is summarized in Alg.~\ref{alg:advance}. In each iteration, we perform time integration and continuous collision detection successively, and handle the earliest collisions if exist, which are discussed in details in the remaining of this section.
%damping
%use current pos and predicted vel
\begin{algorithm}[h]
  \caption{Advance One Step}
  \KwIn{the packed vectors $\bm{q}^n$ and $\dot{\bm{q}}^n$ at the current time and the time step $\Delta t$.}
  \KwOut{the packed vectors $\bm{q}^{n+1}$ and $\dot{\bm{q}}^{n+1}$ after the time step.}
  $t\gets \Delta t$\;
  $\varepsilon_\mathrm{t}\gets \Delta t/25$\;
  \While{$t>0$}{
    $\bm{q}^{n+1},\dot{\bm{q}}^{n+1} \gets$ TimeIntegration($\bm{q}^n,\dot{\bm{q}}^n$)\;
    $colTime \gets$ DetectCollision($\bm{p}^n,\dot{\bm{p}}^{n+1},t,\varepsilon_\mathrm{t}$)\;
    \eIf{$colTime<t$}
    {Roll back to the moment of $colTime$\;
    Handle collisions and update $\bm{q}^{n+1},\dot{\bm{q}}^{n+1}$\;
    $t\gets t - colTime$\;}
    {Break\;}
  }
  \label{alg:advance}
\end{algorithm}
\end{comment}
\subsection{Time Integration}
\label{sec:solver}
Having established spatially discretized equations of motion (Eq.~(\ref{eqn:linear})), we here discuss how to discretize them in time.

We assemble the mass matrix $M\in\mathbb{R}^{12N\times12N}$ according to the component definition in Eq.~(\ref{eqn:mass}).
%satisfying that the $3\times 3$-block starting at $\left(3(I-1),3(J-1)\right)$ takes the value of a third-order identity matrix multiplied by $M^{IJ}$.
The generalized coordinates and the corresponding generalized forces exerted on them are stacked into a $12N$-dimensional $\bm{q}$ and $\bm{F}$ respectively. 
%Computing the right-hand side in Eq.~(\ref{eqn:linear}) gives the 3d generalized force vector applied to the corresponding generalized coordinate. with generalized coordinates stacked into a $12N$-dimensional vector $\bm{q}$ and generalized forces stacked into a $12N$-dimensional vector $\bm{F}$. 
Then Eq.~(\ref{eqn:linear}) is reformulated as 
\begin{equation}
    \bm{M}\ddot{\bm{q}}=\bm{F}\text{.}
\end{equation}
% Since the mass matrix remains constant during the simulation and the stacked vector of generalized forces evolves over time, we write the format of Implicit-Euler time integrator as
It is further discretized by Implicit Euler in time as 
\begin{subnumcases}{\label{eqn:implicit}}
\dot{\bm{q}}^{n+1}=\dot{\bm{q}}^n+\Delta t\,\bm{M}^{-1}\bm{F}(\bm{q}^{n+1},\dot{\bm{q}}^{n+1},t^{n+1})\text{,}\\
\bm{q}^{n+1}=\bm{q}^n+\Delta t\,\dot{\bm{q}}^{n+1}\text{.}
\end{subnumcases}
%The equivalent form obtained by eliminating $\dot{\bm{q}}^{n+1}$ is given by
%\begin{equation}\label{eqn:nonlinear}
%  \bm{h}(\bm{v})=\bm{M}\bm{v}-%\Delta t\,\bm{F}(\bm{q}^{n}+\Delta %t\,\bm{v},\bm{v},t^{n+1})-%\bm{M}\dot{\bm{q}}^n=\bm{0}\text{.}
%\end{equation}
We adopt a Newton's method to solve the above equations iteratively. We refer readers to \S\ref{apx:hessian} for detailed derivation of the Hessian matrix of elasticity energy. \update{We also implement quadratic and cubic line searches referring to the widely used library \emph{ArcSim} \citet{Narain2012,Narain2013}. When facing with ill-conditioned Hessian matrix, we add diagonal regularizers to make it an SPD matrix.}

In practice, for the aforementioned constraints at arbitrary points, we use the augmented Lagragian method \cite{Hestenes1969MultiplierAG} to solve the optimization problem, which acquires better convergence rate than a pure method of Lagrange multipliers.

%To compute the descent direction of $\bm{h}$, the essential step is to compute the Hessian matrix of elasticity, which we refer readers to \S\ref{apx:hessian} for detailed derivation.
%As usual, for quasi-static problems, leaving out the inertia term yields $\bm{F}(\bm{q})=\bm{0}$.

\begin{comment}
% the augmented Lagrangian method
We make specific explanations about the case where boundary conditions are imposed at arbitrary midsurface points. 
% Considering a boundary condition applied at the point $\bm{x}_\mathrm{pt}$ which is expressed as $C(\bm{x}_\mathrm{pt})=0$, augmented Lagrangian method is adopted to solve the constrained optimization problem.
Assuming that all external forces are conservative, then solving Eq.~(\ref{eqn:nonlinear}) is converted into an optimization problem  that $\dot{\bm{q}}^{n+1}=\mathop{\arg\min}_{\bm{v}}E(\bm{v})\text{,}$
where $\bm{h}(\bm{v}) = \mathrm{d} E(\bm{v})/\mathrm{d}\bm{v}$. 
Denoting the constraints by $\bm{C}(\dot{\bm{q}})=0$, 
% taking $\frac{\mathrm{d}\bm{q}}{\mathrm{d}\dot{\bm{q}}}$,
the constrained optimization problem, with $\bm{\eta}$ as the Lagrange multipliers and $c$ as the penalty coefficient, is formulated as 
\begin{equation}
    \dot{\bm{q}}^{n+1}=\mathop{\arg\min}_{\bm{v}}E(\bm{v})+\bm{\eta}\cdot\bm{C}(\bm{v})+\frac{c}{2}{\mathop{||}\bm{C}(\bm{v})\mathop{||}}_2^2\text{,}
\end{equation}  
according to the augmented Lagrangian method \cite{}, which is then solved by alternating updates. 
% Since $\bm{C}(\dot{\bm{q}})$ is w.r.t. $\dot{\bm{q}}$, $\nabla\bm{C}$ is a constant vector independent of $\dot{\bm{q}}$.
% Then $\bm{q}^{n+1}$ is solved from the linear equations
% \begin{equation}
%     \bm{h}(\dot{\bm{q}})+\bm{\eta}\nabla\bm{C}=\bm{0}
% \end{equation}
% iteratively. In each iteration, given $\bm{\eta}$, we utilized a Newton solver to obtain a $\bm{q}^{n+1}$ and check whether $\bm{C}(\dot{\bm{q}})=\bm{0}$ is satisfied within some error threshold. If not, $\bm{\eta}$ is doubled and we go to the next iteration. Otherwise we take the $\bm{q}^{n+1}$ as the final result.
\end{comment}

\subsection{Collision Detection}
We utilize the point-to-surface intersection detection scheme for continuous collision detection. 
In practical implementation, the sampling strategy is adjusted to specific scenarios.
%We point out that CCD problems of surfaces are converted into point-to-patch intersection detetion through sampling strategy which is adjusted to specific scenarios.
For collision detection between shell and colliders with simple geometry shape, such as spheres, cylinders or planes, the midsurface is uniformly sampled. 
%To detect collisions between a thin shell and a collider with simple geometry that has a closed form of signed distance function, e.g., a sphere or an infinite plane, we sample the shell midsurface and CCD can be easily done between the sampling points and the geometry.
As for the collision detection with colliders possessing complex shapes, we sample the collider surface, or directly take the surface vertices as the sample points, if the collider has a triangular mesh.
%and detect continuous intersection of the sampling points and the patches of the shell midsurface. If the collider is modeled by an explicit representation like triangle mesh, the sampling points can be taken as the vertices of the collider. 
For the thin shell self-collision, we iteratively sample each B\'{e}zier surface, and perform the continuous collision detection on sampling points against all the other surfaces. Penetrations occurring within a single surface can be handled by subdividing the current surface with the scheme illustrated in Fig.~\ref{fig:subany} and treating the $4$ subdivided regions recursively.
%We found penetration within a single patch rarely happens in all of our examples.

%leaving out the square neighborhood of the sampling point and detect collisions of the point with the remaining region which is then divided into 4 patches as illustrated in Fig.~(\ref{})
%sample each patch of its midsurface and detect continuous intersection of all the other patches of midsurface with it. 
%Though penetrations may occur within a single patch, 

%it rarely happens in all our simulations. Nevertheless, one can detect this kind of collision by a similar idea used in \S\ref{sec:render} --- we leave out the square neighborhood of the sampling point and detect collisions of the point with the remaining region which is then divided into 4 patches as illustrated in Fig.~(\ref{}).

% An individual collision event is modeled as the a collision between a pair of points. 
% We have elaborated the algorithm of detecting such a collision event that occurs earliest in a time step, 
%For robust and rapid collision handling, we pick a set of collisions that occur at almost the same time. These collisions are resolved simultaneously by the algorithm described in the following text.
% This means to 
% As is summarized in Algorithm.~(\ref{alg:ccd}), 
%Specifically, we sample $4^2$ points uniformly in each patch, 
% leaving out the common edge and shell boundaries which may introduce numerical issues.
% \xw{no special treatment for boundaries?}
%and adopt the sampling strategies described above
% to convert the CCD problem into a series of investigation of point-to-surface intersection. 
%when looping to check all the point-surface pairs in each iteration, we perform the continuous point-to-surface intersection detection.
%if a collision occurs no later than a certain threshold $\varepsilon_\mathrm{t}$ compared to the moment of the detected earliest collision, we add it to the collision list and update the collision moment.
% We traverse the patches of the midsurface to utilize continuous ray-surface intersection algorithm for continuous collision detection, inside each iteration of which, we record all the collisions within $colTime+\varepsilon_\mathrm{t}$ in $colList$ and update $colTime$
% We relax the pruning condition in \S\ref{sec:render} by a certain time threshold within a time threshold after the detected earliest time.
%Once the loop check is done and collisions exist, we sort the collision list by time of occurrence in ascending order. The collision moment is set as the time of occurrence of the first element in the list, and collisions that occur later than $\varepsilon_\mathrm{t}$ after the collision moment are discarded. 

\begin{comment}
\begin{algorithm}[h]
  \caption{Detect Collision}
  \KwIn{the packed vectors $\bm{q}$ and $\dot{\bm{q}}$, the upperbound of the collision time $t$ and the threshold $\varepsilon_\mathrm{t}$}
  \KwOut{the list of simultaneous collisions $colList$ and the earliest time $colTime$ of collisions.}
  Empty $colList$\;
  $colTime\gets t$\;
  \For{each patch of the midsurface}{
    \For{each sampling point}{
        \For{each of the colliders and the rest patches}{
            Detect intersections by algorithm described in \S\ref{sec:ccd} within $colTime+\varepsilon_\mathrm{t}$\;
            \uIf{intersections detected}{
                Add collisions into $colList$\;
                Update $colTime$\;
            }
        }
    }
  }
  Detect and record self-collisions within $colTime+\varepsilon_\mathrm{t}$ in $colList$ and update $colTime$\;
  Detect and record cloth-to-collider collisions within $colTime+\varepsilon_\mathrm{t}$ in $colList$ and update $colTime$\;
  \uIf{$colList$ is not empty}{
    Sort $colList$ by time of occurrence in ascending order\;
    $colTime \gets$ the time of occurrence of the first element in $colList$\;
    Discard the collisions that occur after $colTime + \varepsilon_\mathrm{t}$;
  }
  Return $colTime$\;
  \label{alg:detect}
\end{algorithm}
\end{comment}

\subsection{Collision Handling}
We roll back the system to the collision moment, which prohibits penetration throughout the simulation. Then the detected collisions are going to be handled in one batch. Using a zero restitution coefficient uniformly for collisions \cite{Bridson2002}, the change of velocities of each collision points are computed according to the conservation of momentum. 
An impulse-based method is used to compute the instantaneous collision response, with each collision modeled as a constraint \cite{Vouga08}.

Considering a single collision point $\bm{x}_\mathrm{c}$ with its normal velocity after the collision $v_\mathrm{nc}$, the constraint is expressed as $C=\bm{n}_\mathrm{c}\cdot\dot{\bm{x}}'_\mathrm{c}-v_\mathrm{nc}=0$, where we use a prime to denote the quantities after collision handling. It is noteworthy that this constraint is linear to the generalized velocities, which means it can be reformulated as
\begin{equation}
    C=\nabla C\cdot\dot{\bm{q}}'-v_\mathrm{nc}=0\text{,}
    \label{eqn:constraint}
\end{equation}
The impulse exerted on the point is supposed to be along the derivative of the constraint with a certain magnitude $\eta$, which can be formulated as $\bm{M}(\dot{\bm{q}}'_\mathrm{c}-\dot{\bm{q}}_\mathrm{c})=\eta\nabla C$. Thus we obtain 
\begin{equation}
    \dot{\bm{q}}'_\mathrm{c}=\dot{\bm{q}}_\mathrm{c}+\eta\bm{M}^{-1}\nabla C\text{.}
    \label{eqn:impulse}
\end{equation}
Substituting Eq.~(\ref{eqn:impulse}) into Eq.~(\ref{eqn:constraint}) yields a one-variable equation about $\eta$, which is then solved, as
\begin{equation}
    \eta = \frac{-\nabla C\cdot\dot{\bm{q}}+v_\mathrm{nc}}{(\nabla C)^\mathrm{T}\bm{M}^{-1}\nabla C}\text{.}
    \label{eqn:impulsemag}
\end{equation}
The updated velocity is acquired by substituting $\eta$ into Eq.~(\ref{eqn:impulse}).

Consequently, when solving for multiple collision points simultaneously, Eq.~(\ref{eqn:impulsemag}) expands to its vector form as:
\begin{equation}
    \left((\nabla \bm{C})^\mathrm{T}\bm{M}^{-1}\nabla \bm{C}\right)\bm{\eta} = -\nabla \bm{C}\cdot\dot{\bm{q}}+\bm{v}_\mathrm{nc}\text{,}
\end{equation}
with a vector $\bm{C}=(\nabla \bm{C})^\mathrm{T}\dot{\bm{q}}'-\bm{v}_\mathrm{nc}=\bm{0}$ and a vector $\bm{\eta}$.
% a vector C with one component per constraint and a vector $\bm{\eta}$ with one component per point.
\begin{comment}
Furthermore, multiple collision points introduce multiple constraints that are stacked into a vector $\bm{C}=(\nabla \bm{C})^\mathrm{T}\dot{\bm{q}}'-\bm{v}_\mathrm{nc}=\bm{0}$, with each component denoting a constraint from one point. This requires a $\bm{\eta}$ vector, with each component for one constraint. The expressions can be obtained through similar derivation, resulting in the equations of $\bm{\eta}$ by
\begin{equation}
    \left((\nabla \bm{C})^\mathrm{T}\bm{M}^{-1}\nabla \bm{C}\right)\bm{\eta} = -\nabla \bm{C}\cdot\dot{\bm{q}}+\bm{v}_\mathrm{nc}\text{.}
\end{equation}
\end{comment}
It is worth noticing that since the matrix can be linearly correlated, in practice we are solving for $\bm{\eta}$ in a least-squares sense. 

Merely updating velocity at a collision point would result in the same collision being detected at the beginning of the next round of CCD, 
which can not be distinguished according to the direction of relative velocity because of the particularity of shells.
We therefore push out each collision point a subtle distance $\varepsilon_\mathrm{d}$ ($10^{-4}$ in practice) opposite the normal direction, which can also be viewed as letting the point move along the change in velocity for a subtle while.
A push-out applied on a single collision point is also modeled as a constraint that says $C=\bm{n}_\mathrm{c}\cdot\bm{x}'_\mathrm{c}-\varepsilon_\mathrm{d}=0$. The position constraints applied on multiple collision points are resolved using the same scheme as velocity constraints.

% There are possibilities that new collisions are introduced when resolving the existing ones,

\update{
We handle frictional contact in a similar way by rewriting the constraint $C$ in Eq.~(\ref{eqn:constraint}) with frictional impulse taken into account. 
According to the Coulomb friction cone, we compute the applied frictional impulse on the tangent direction of the collision point. Then we extend Eq.~(\ref{eqn:constraint}) which constrains only the normal component of the velocity update to constraining both normal and tangent component updates. The subsequent process is the same as above, with the only difference being the dimension of the constraints.
}

==> Sections-old/Intersection.tex <==
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[2]{\begin{subfigure}{0.196\linewidth}\centering\includegraphics[trim=0.75cm 1cm 2.5cm 0.5cm,clip,width=\textwidth]{#1}\caption{#2}\vspace{-0.3cm}\end{subfigure}}
    \centering
    \formattedgraphics{Figures/teapot/teapot-mesh1.png}{265 vertices;}
    \formattedgraphics{Figures/teapot/teapot-mesh2.png}{1,041 vertices;}
    \formattedgraphics{Figures/teapot/teapot-mesh3.png}{4,129 vertices;}
    \formattedgraphics{Figures/teapot/teapot-mesh4.png}{16,449 vertices;}
    \formattedgraphics{Figures/teapot/teapot-bezier.png}{32 patches.}
    \caption{Parametric surface rendering. A Utah teapot represented in bicubic patches is rendered by our scheme, shown in (e). The teapots rendered by traditional methods with each patch triangulated into 4/16/64/256 facets are shown in (a)/(b)/(c)/(d), where artifacts can be seen at the mouth and silhouettes the teapots, especially for coarse mesh decimation. }
    \label{fig:teapot}
    \vspace{-0.3cm}
\end{figure*}
\section{Surface Intersection Detection}

%We then develop algorithms for rendering and collision handling. We model both these situations as surface element intersection problems and solve them within the same framework based on subdivision. The main difference is whether the surface moves over time. In this section, we will elaborate our solutions successively.

As previously described, the shape functions of BH elements are defined as tensor products of cubic polynomials with real coefficients.
Therefore, We can equivalently transform a BH surface into a B\'{e}zier surface by regarding these polynomials as a linear combination of \emph{Bernstein basis polynomials} of degree $3$: 
\begin{equation}
  \bm{x}(\xi^1,\xi^2)=\sum_{i=0}^3\sum_{j=0}^3B^i(\xi^1)B^j(\xi^2)\bm{p}_{ij}\text{,}
\end{equation}
where $B^i(x)$ is defined as $\tbinom{3}{i}x^i(1-x)^{3-i}$ and $\bm{p}_{ij}\in \mathbb{R}^3$ denote control points.
A B\'{e}zier form provides us with a strong property that a surface lies completely within the convex hull of its control points, and thus also completely within the bounding box of its control points in any given Cartesian coordinate system, which lays the foundation of our ray-surface intersection detection algorithms.

Surface intersection is an important geometric operation in CAGD, we mainly focus on finding the intersection point of ray and surface in this paper. According to whether the surface moves during ray propagation, two kinds of intersections can be detected, which allows both ray-tracing rendering (surfaces fixed) and continuous collision detection (surfaces movable).
\begin{figure}
\begin{subfigure}{0.495\linewidth}
\begin{tikzpicture}
	\draw[step=2] (0,0) grid (2,2);
	\draw (0,1)--(2,1);
	\draw (1,0)--(1,2);
	\fill (0,0) circle (0.05);
    \fill (0,2) circle (0.05);
    \fill (2,0) circle (0.05);
    \fill (2,2) circle (0.05);
	\node at(-0.2,-0.3) {$(u_\mathrm{min},v_\mathrm{min})$};
    \node at(2.2,2.3) {$(u_\mathrm{max},v_\mathrm{max})$};
    \node at(-0.2,2.3) {$(u_\mathrm{min},v_\mathrm{max})$};
    \node at(2.2,-0.3) {$(u_\mathrm{max},v_\mathrm{min})$};
    \node at(0.5,1.5) {1};
    \node at(1.5,1.5) {2};
    \node at(0.5,0.5) {3};
    \node at(1.5,0.5) {4};
\end{tikzpicture}
\caption{}
\label{fig:submid}
\end{subfigure}
\begin{subfigure}{0.495\linewidth}
\begin{tikzpicture}
	\draw[step=2] (0,0) grid (2,2);
	\fill (1.4,0.8) circle (0.05);
	\draw (1.2,0.6)--(1.2,2);
	\draw (1.6,0.6)--(0,0.6);
	\draw (1.6,1)--(1.6,0);
	\draw (1.2,1)--(2,1);
	\fill (0,0) circle (0.05);
    \fill (0,2) circle (0.05);
    \fill (2,0) circle (0.05);
    \fill (2,2) circle (0.05);
	\node at(-0.2,-0.3) {$(u_\mathrm{min},v_\mathrm{min})$};
    \node at(2.2,2.3) {$(u_\mathrm{max},v_\mathrm{max})$};
    \node at(-0.2,2.3) {$(u_\mathrm{min},v_\mathrm{max})$};
    \node at(2.2,-0.3) {$(u_\mathrm{max},v_\mathrm{min})$};
    \node at(0.6,1.3) {1};
    \node at(1.6,1.5) {2};
    \node at(0.8,0.3) {3};
    \node at(1.8,0.5) {4};
\end{tikzpicture}
\caption{}
\label{fig:subany}
\end{subfigure}
\caption{Ray surface intersection subdivide schemes. Left: splitting at midpoint; Right: abandoning the neighborhood of intersection point and splitting the rest region.}
\vspace{-0.3cm}
\end{figure}
\subsection{Static Intersection Detection}
\label{sec:render}
%1. statement of ray intersection problem
%2. brief description of de Casteljau algorithm (how to divide a patch), convex hull property (how to get bounding box) and heap structure
%3. step 1, perform coordinate transform to make ray in z axis
%4. step 2, using heap to generate online BVH
%5. step 3, if the top of heap is not small enough, subdivide into four pieces(with Fig)
%6. using Newton's method to prune during step 3(with Fig)
%Our ray-surface intersection algorithm utilizes the property of B\'ezier patch to generate online BVH along with Newton's method to prune. We use a heap data structure to record the nearest subdivided patch to the ray.
%Casteljau algorithm

In a ray-tracing rendering framework, the most expensive part is to test whether, where, and when a ray intersects the object.
In order to accelerate intersection tests, a conventional solution for triangular meshes is to build a BVH tree in advance.
Our algorithm for B\'{e}zier surfaces do not require any tree construction, with bounding volume hierarchies generated heuristically and implicitly for each ray.

Supposed that a ray is defined by
\begin{equation}
  \bm{x}_\mathrm{ray}(\tau) = \bm{x}_\mathrm{0} + \tau\bm{d}\text{,}
  \label{eqn:ray}
\end{equation}
where $\bm{d}$ indicates the direction and $\tau$ denotes the (pseudo) time, the task in intersection tests is to find $(\xi^1,\xi^2)$ and minimum $\tau>0$ such that $\bm{x}_\mathrm{ray}(\tau)=\bm{x}(\xi^1,\xi^2)$ holds.
For any $\xi^1$, $\xi^2$, and $\tau$ that satisfy this intersection equation, the convex-hull property of B\'{e}zier surfaces suggests us
\begin{equation}
  \min_{i,j\in\{0,1,2,3\}}\left\{\bm{p}_{ij}\cdot\hat{\bm{e}}_k\right\}\le(\bm{x}_0+\tau\bm{d})\cdot\hat{\bm{e}}_k\le\max_{i,j\in\{0,1,2,3\}}\left\{\bm{p}_{ij}\cdot\hat{\bm{e}}_k\right\}\text{,}
  \label{eqn:ineqray}
\end{equation}
with $\hat{\bm{e}}_k$ ($k\in\{1,2,3\}$) denoting the $k$-th vector of the standard basis.
Actually, this is equivalent to an intersection test between the ray and an axis-aligned bounding box (AABB),
which implies $6$ inequalities. Solving (\ref{eqn:ineqray}) for $\tau$, we can either acquire an interval $[\tau_\mathrm{min},\tau_\mathrm{max}]$ or prove that no $\tau>0$ satisfy all the inequalities.
If faced with the latter case, we conclude that the current surface is not intersected by the ray and turn to another surface with safety.

When the former case is encountered after solving (\ref{eqn:ineqray}), a divide-and-conquer strategy is used.
By splitting a B\'{e}zier surface into four smaller B\'{e}zier surfaces with De Casteljau's algorithm \cite{BOEHM1999587} at specific parameter coordinates, we can recursively perform ray-AABB tests and discard surfaces that are impossibly intersected by the ray.
Finally, we either discard all surfaces or obtain an arbitrarily small interval of $\tau$.
In practice, with $[u_\mathrm{min},u_\mathrm{max}]$ and $[v_\mathrm{min},v_\mathrm{max}]$ respectively denoting the intervals of $\xi^1$ and $\xi^2$ for every surface, we terminate the algorithm if the ray intersects the AABB of a surface and both $(u_\mathrm{max}-u_\mathrm{min})$ and $(v_\mathrm{max}-v_\mathrm{min})$ are less than some threshold.

This subdivision-based algorithm is trivial but effective and robust, which converges to the accurate intersection point linearly.
Since the ray might intersect with the surface at multiple points, but only the closet one is required for the algorithm, in order to limit the number of surfaces that need to be checked for collision, 
we improve the process of choosing the next surface by a min heap of candidate surfaces. Every time a new surface is generated, we push it into the heap with $\tau_\mathrm{min}$ as the key for sorting, and every time we turn to another surface, the heap top is chosen.
It is clear that the first considered surface that meets the termination condition gives an accurate approximation of the minimum $\tau$, among all the intersection points.

Last but not least, a Newton's method is used to decide where to subdivide surfaces by solving $\bm{x}(\xi^1,\xi^2)=\bm{x}_\mathrm{ray}(\tau)$ directly. 
Whenever a surface is going to be subdivided, we set the central parameter coordinates of it as the initial guess.
Within a fixed number of iterations, if the Newton's method 
converges to $\xi^1\in[u_\mathrm{min},u_\mathrm{max}]$ and $\xi^2\in[v_\mathrm{min},v_\mathrm{max}]$, we obtain an intersection point and use the corresponding $\tau$ to update the current optimal solution $\tau_\mathrm{opt}$ if $\tau$ is smaller and positive. 
The found intersection point may not be the closest one, but we can remove it from the search space by abandoning
%Then, we abandon 
the neighbourhood of $(\xi^1,\xi^2)$ in the parameter space and subdividing the other region as illustrated in Fig.~\ref{fig:subany}. If the Newton's method does not converge, we split the surface as usual from the midpoint (Fig.~\ref{fig:submid}).
%does not converge with $\xi^1\in[u_\mathrm{min},u_\mathrm{max}]$ and $\xi^2\in[v_\mathrm{min},v_\mathrm{max}]$, no extra information is acquired and we have to split the surface as usual. If converged, we obtain an intersection point and use the corresponding $\tau$ to update the optimal solution. In this situation, we abandon the neighbourhood of $(\xi^1,\xi^2)$ in the parameter space and subdivide the other region as illustrated in Fig.~\ref{}. 

These two improvements lead to a great acceleration for the subdivision-based algorithm, resulting in even faster performance than a theoretically quadratic-convergent algorithm, such as B\'{e}zier clipping, as shown in Tab.~\ref{tab:performance} and Fig.~\ref{fig:performance}. The algorithm optimized by Newton's method, summarized in Alg.~\ref{alg:render}, shows the best in efficiency over three scenes.

\begin{comment}
Step 1. We perform coordinate transformation to change the ray's origin to the origin in the world space and ray's direction to the positive z axis. Suppose the B\'ezier patch in this coordinate is $\bm{S}(u,v)$.

Step 2. We use a heap data structure to record the nearest patch. The heap is ranked in the signed distance of ray to heap's bounding box. We apply convex hull property to get the bounding box of the patch. If the bounding box of the patch is not intersect with ray, the patch itself won't have intersection. Otherwise, we push the patch into the heap.

Step 3. If the heap is not empty. We get the patch from top of the heap. If the size of patch in each parametric direction is smaller than a threshold, that is $\Delta\xi^1, \Delta\xi^2<\epsilon$, we choose the center of the current parameter subdomain as intersection point.
\begin{equation}
	(\xi^1, \xi^2) = \frac{1}{2}(\xi^1_{\min}+\xi^1_{\max},\xi^2_{\min}+\xi^2_{\max})
\end{equation}
This intersection point might not be the nearest, so we must record it and keep subdividing. Every time we find a intersection point, we update the information of nearest intersection. We use the known intersection point to prune. If the distance from the ray to a patch's bounding box is far from it to that point, we can discard the patch. 

If the patch is not small enough, we apply de Casteljau algorithm to subdivide this patch evenly into four pieces shown as Fig(??). These subdivided patches go through step 2 to decide whether they should push into the heap. We stay in step 3 until the heap is not empty.

Step 4. If the heap is empty, the recorded intersection point is the nearest point. If no intersection point is recorded then the ray patch do not intersect.

\xw{tbd: a brief proof of convergence}
% We can use Newton's method to find intersection point faster during step 3. We solve the equations $S_x(\xi^1,\xi^2)=0, S_y(\xi^1,\xi^2)=0$ with fixed steps of Newton iteration. If the Newton's method converges, that is $(\xi^1,\xi^2)$ belongs to patch's parametric domain and $S_z(\xi^1,\xi^2)>0$, we find a intersection point. We also change the way of subdivision shown in Fig(??)

To accelerate the process of finding an intersection point in step 3, we use Newton's method to solve the equations $S_x(\xi^1,\xi^2)=0, S_y(\xi^1,\xi^2)=0$ with a fixed number of iterations. If the Newton's method converges to a point $(\xi^1,\xi^2)$ that satisfies $S_z(\xi^1,\xi^2)>0$ within the parametric domain of the patch, an intersection point is found.

A better way of subdivision is to the abandon a tiny box containing the point found by Newton's method and divide the rest of the patch as depicted in Fig.~(\ref{}). 
\end{comment}
\begin{figure}
    \centering
    \begin{minipage}[h]{\linewidth}
        \centering
        \captionsetup*{type = table}
        \caption{Rendering performance. The three algorithms from left to right are: our subdivision-based that split only  at the midpoint, our algorithm with Newton's method, and B\'{e}zier clipping.}
        %\captionof{table}{\cheng{Rendering performance. Three algorithm from left to right are our subdivision-based algorithm that only splitting at midpoint, our algorithm with Newton's method, and B\'{e}zier clipping.}}
        \begin{tabular}{|c|c|c|c|} \hline
                &  Subdivision &  Subdivision (Opt.) &B\'ezier clipping\\ \hline
        Plane    & $\SI{58.3}{\second}$ & $\SI{4.5}{\second}$  & $\SI{6.0}{\second}$\\ \hline
        Cylinder & $\SI{91.6}{\second}$ & $\SI{9.7}{\second}$  & $\SI{14.2}{\second}$\\ \hline
        Drape    & $\SI{86.0}{\second}$ & $\SI{14.8}{\second}$ & $\SI{33.9}{\second}$\\ \hline
        \end{tabular}
        \label{tab:performance}
    \end{minipage}
    \begin{minipage}[h]{\linewidth}
        \centering
    \begin{annotationimage}{trim=0cm 0cm 0cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/plane.png}
        \draw[coordinate label = {Plane at (0.138,0.07)}];
    \end{annotationimage}
    \begin{annotationimage}{trim=3.5cm 0cm 3.5cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/cylinder.png}
        \draw[coordinate label = {Cylinder at (0.195,0.08)}];
    \end{annotationimage}
    \begin{annotationimage}{trim=3.5cm 0cm 3.5cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/drape.png}
        \draw[coordinate label = {Drape at (0.15,0.08)}];
    \end{annotationimage}
    \caption{Three test cases with only 1 patch for Plane and $10\times10$ patches for Cylinder and Drape each. The scenes all have the same setting of lights and 16 samples per pixel.}
    \label{fig:performance}
    \end{minipage}
\end{figure}
% \begin{table}[h]
%     \caption{rendering performance}
%     \begin{tabular}{|c|c|c|c|} \hline
%                         &  subdivision &  subdivision + Newton &B\'ezier Clipping\\ \hline
%         plane             &    58.3 &  4.5  & 6.0             \\ \hline
%         cylinder            &    91.6 &  9.7  & 14.2           \\ \hline
%         drape     &    86.0 &  14.8 & 33.9           \\ \hline
%     \end{tabular}
%     \label{tab:performance}
% \end{table}
% \begin{figure}[t]
%     \centering
%     \begin{annotationimage}{trim=0cm 0cm 0cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/plane.png}
%         \draw[coordinate label = {Plane at (0.138,0.07)}];
%     \end{annotationimage}
%     \begin{annotationimage}{trim=3.5cm 0cm 3.5cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/cylinder.png}
%         \draw[coordinate label = {Cylinder at (0.195,0.08)}];
%     \end{annotationimage}
%     \begin{annotationimage}{trim=3.5cm 0cm 3.5cm 0cm,clip,width = 0.322\linewidth}{Figures/render_performance/drape.png}
%         \draw[coordinate label = {Drape at (0.15,0.08)}];
%     \end{annotationimage}
%     \caption{performance}
%     \label{fig:performance}
% \end{figure}


\begin{algorithm}[htbp]
  \caption{Static Intersecting Detection}
    \SetKwFunction{IntersectsAABB}{IntersectsAABB}
    \SetKw{KwBreak}{break} 
    \SetKw{KwNull}{null} 
    \KwIn{The ray $\bm{x}_\mathrm{ray}$ and the surface.}
    \KwOut{The nearest intersection point $(\xi^1,\xi^2)$ or null indicating no intersecion.}
    $\tau_\mathrm{opt}\gets\infty$\;
    Construct a min heap\;
    \eIf {\IntersectsAABB{$\bm{x}_\mathrm{ray}$, the whole surface}}
    {Push the whole surface into the heap with its $\tau_{\min}$ as the key\;}{\Return null\;}
    \While{the heap is not empty}{
        $\text{The current surface}\gets$ the top of the heap\;
        \lIf{$\tau_{\min} > \tau_\mathrm{opt}$}{\KwBreak}
        \If{the surface is small enough}{
            \Return the middle parameter coordinates of the surface\;
        }
        Find an intersection point by Newton's method\;
        \eIf{converged}{
            Update $\tau_\mathrm{opt}$ and $(\xi^1_\mathrm{opt},\xi^2_\mathrm{opt})$\;
            Subdivide the surface by the scheme in Fig.~\ref{fig:subany}\;
        }{
            Subdivide the surface by the scheme in Fig.~\ref{fig:submid}\;
        }
        \ForEach{subdivided surface}{
            \If{\IntersectsAABB{$\bm{x}_\mathrm{ray}$, the subdivided surface}}{
                Push the surface into the heap with its $\tau_{\min}$ as the key\;
            }
        }
    }
    \eIf{$\tau_\mathrm{opt} \neq +\infty$}{\Return $(\xi^1_\mathrm{opt},\xi^2_\mathrm{opt})$\;}{\Return null\;}
     \label{alg:render}
\end{algorithm}
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[2]{\begin{subfigure}{0.196\linewidth}\centering\includegraphics[trim=0cm 0cm 0cm 0cm,clip,width=\textwidth]{#1}\caption{#2}\vspace{-0.3cm}\end{subfigure}}
    \centering
    \formattedgraphics{Figures/caustic/caustic-mesh1.png}{3,160 vertices;}
    \formattedgraphics{Figures/caustic/caustic-mesh2.png}{14,520 vertices;}
    \formattedgraphics{Figures/caustic/caustic-mesh3.png}{57,840 vertices;}
    \formattedgraphics{Figures/caustic/caustic-mesh4.png}{230,880 vertices;}
    \formattedgraphics{Figures/caustic/caustic-bezier.png}{450 patches.}
    \caption{Parametric surface rendering. The caustic lighting effect amplifies the imperfection of the surface, such as the un-smooth surface normal distribution. Fine-grained caustic rays clutter the ground for the scenarios with low resolution mesh object. 
    %A caustic bottle cup with uneven surface rendered using BHEM is shown in (e). After the surface triangulated in the same way as those in Fig.~\ref{fig:teapot}, fine-grained caustic rays are cluttered on the ground.
    }
    \label{fig:caustic}
    \vspace{-0.3cm}
\end{figure*}
\subsection{Continuous Intersection Detection}
\label{sec:ccd}
Continuous collision detection aims at finding the earliest intersection point between moving objects. Concentrating on the intersections between a surface and other objects, as well as self-intersections of the surface, 
we employ a point-to-surface detection scheme where points (sampled from the objects) are tested for trajectory intersection against a moving surface.

Supposed that the velocity keeps constant within a single time step $\Delta t$, a time-varying B\'{e}zier surface is given by
\begin{equation}
	\bm{x}(\xi^1,\xi^2,t)=\sum_{i=0}^3\sum_{j=0}^3B_i^3(\xi^1)B_j^3(\xi^2)(\bm{p}_{ij}+t\dot{\bm{p}}_{ij})\text{,}
\end{equation}
where $\bm{p}_{ij}$ and $\dot{\bm{p}}_{ij}$ are the initial position and velocity of the $(i,j)$-th control point, and $t\in[0,\Delta t]$ indicates the time. The trajectory of a moving point can be depicted
%given in the same form (Eq.~(\ref{eqn:ray})) 
as a parameterized ray as
\begin{equation}
    \bm{x}_\mathrm{p}(t)=\bm{x}_\mathrm{p0}+t\dot{\bm{x}}_\mathrm{p}\text{,}
\end{equation}
where $\bm{x}_\mathrm{p0}$ and $\dot{\bm{x}}_\mathrm{p}$ denote the initial position and velocity of the point.

Still according to the convex-hull property, a necessary condition for the intersection to occur at the moment $t$ is that the point is inside the axis-aligned bounding box of the surface at that very moment, which can be written as
{\footnotesize%
\begin{equation}
    \min_{i,j}
    \left\{(\bm{p}_{ij}+t\dot{\bm{p}}_{ij})\cdot\hat{\bm{e}}_k\right\}
    \le (\bm{x}_\mathrm{p0}+t\dot{\bm{x}}_\mathrm{p})\cdot\hat{\bm{e}}_k
    \le \max_{i,j}\left\{(\bm{p}_{ij}+t\dot{\bm{p}}_{ij})\cdot\hat{\bm{e}}_k\right\}\text{,}
    \label{eqn:ineqccd}
\end{equation}}%
with $i,j\in\{0,1,2,3\}$. 
If we can solve (\ref{eqn:ineqccd}) for $t$, just as that done in \S\ref{sec:render} for $\tau$, a similar subdivision-based algorithm can also be utilized here.
%Then the task is to solve for $(\xi^1,\xi^2)$ and the minimum $t\in[0,\Delta t]$ that satisfies the above inequalities.

%The difference between Eq.~(\ref{eqn:ineqccd}) and Eq.~(\ref{eqn:ineqray}) lies in the LHS and RHS which are no longer known scalar quantities. 
For each inequality on the left-hand side, the result is equivalent to the union of the intervals solved from the inequalities
\begin{equation}
  (\bm{p}_{ij}+t\dot{\bm{p}}_{ij})\cdot\hat{\bm{e}}_k\le(\bm{x}_\mathrm{p0}+t\dot{\bm{x}}_\mathrm{p})\cdot\hat{\bm{e}}_k\text{,}
\end{equation}
where $i$ and $j$ ranges in $\{0,1,2,3\}$. The same interpretation holds for the right-hand side of (\ref{eqn:ineqccd}). The solution of (\ref{eqn:ineqccd}) is the intersection of the two unions, which can be solved by segment-tree or greedy algorithms. 
If there exists no feasible solution inside $[0,\Delta t]$, then no intersection occurs in the time step.
Otherwise, we can adopt the divide-and-conquer framework described in \S\ref{sec:render} to detect possible intersection recursively.
Similarly, a Newton's method can be used to decide how to subdivide surfaces and accelerate convergence.


==> Sections-old/Introduction.tex <==
\section{Introduction}

%Shell is one of the vital structures that make up the world, from soft cloth to stiff car hull, from nanometer-sized cell membranes to kilometer-scale crusts.Among them, 
A thin shell structure specifically refers to an object
%a shell structure 
whose thickness is sufficiently small compared to its other two dimensions, such as cloth, paper, aircraft fuselage. 
%Thin-shell objects, such as cloth, Origami, balloon, aircraft fuselage, often exhibit special performance such as high strength-to-weight and stiffness-to-weight ratios, and excellent design flexibility. Owing to their wide applications, great efforts have been made to the development of advanced theoretical models to accurately and efficiently predict the deflection behaviors of them in the computational physics field.
The Kirchhoff--Love (KL) theory \cite{Ciarlet2000} is commonly invoked to describe the mechanical behavior of thin shells. 
Kirchhoff--Love assumes that the transverse shear is negligible throughout the deformation and thus the shell kinetics is adequately described by \emph{midsurface}'s in-plane stretching and lateral bending.
%Assuming that any transverse normal remains perpendicular to the \emph{midsurface} throughout deformation, the problem of studying deformation of a 3D shell volume can be attractively simplified to that of its midsurface (a 2D surface); the shell kinetics is then  described as in-plane stretching and lateral bending.
%Accordingly to the KL assumption, only the midsurface is adequate for representing and simulating the overall shell volume.

%In computer graphics, this reduced model has gained great attentions as well and being employed for cloth \cite{}, skin \cite{}, and paper \cite{} simulation based on linear finite element methods. 
In computer graphics, 
%the shell midsurface geometry is usually represented as triangle meshes, and is simulated using linear finite elements.
taking Lagrange interpolation polynomials as the basis functions in finite-element analysis is an overwhelmingly popular choice today. However, it is difficult to achieve $\mathcal{C}^1$-continuity in element interface, which makes the bending energy not everywhere well defined in the domain. 
%between elements is difficult to achieve in Lagrangian-based finite element interpolation, such as the most popular linear finite element based The most critical problem of this linear scheme is that the solution's $\mathcal{C}^1$ continuity required for solving the equations of motion with the Galerkin method can not be satisfied \cite{}.
%The critical problem of the linear triangular element is that only $\mathcal{C}^0$ continuity is ensured in the element interface, and this is unable to meet the $\mathcal{C}^1$ continuity requirement for discretizing the weak form of KL model.
This is because the KL model features a curvature-based bending energy model, which corresponds to the term involving second-order derivatives of displacements in its weak form PDE. $\mathcal{C}^1$-continuity requires that finite element solution and its first‐ and second‐order derivatives must be square-integrable.

A conventional solution is to decouple the non-integrable bending energy from membrane energy, and designate the discrete definition of the bending energy as a specific function of the dihedral angle according to discrete differential geometry \cite{Bridson2002,Grinspun2003,Bergou2006}. 
However, this approach implies that the shell can only bend along common edges of elements, which leads to severe locking issue~\cite{Chen2018,Quaglino2016}, most prominent when the shell is extremely thin, or inextensible constraint is enforced. 
%Using extremely high resolution triangular meshes \cite{}, runtime remeshing \cite{}, treating inextensibility as a hard constraint \cite{} can circumvent the locking effects by sacrificing computation efficiency and accuracy. 
%cannot guarantee that the bending strain will arrive at the true solution as the geometry is meshed more finely. 
Subdividing finite elements~\cite{Cirak2000,Guo2018,Clyde2017} provides a viable strategy for satisfying higher regularity for midsurface interpolation functions in FEM solution. But the resulting basis functions obtained with subdivision surfaces are non-polynomial and non-interpolating, which complicates both numerical integration and collision handling, as latter needed. 

Isogeometric Analysis (IGA)~\cite{Hughes2005, Cottrell2009} is an appealing alternative to 
%the integration of geometric modeling and shell analysis, 
attaining high order continuity solution space.
It utilizes various basis functions emanating from computer aided geometric design (CAGD) in finite element analysis, such as B-splines~\cite{Hollig2012} and NURBS~\cite{Qin1994, Lu2014, Trusty2021} for their global smoothness. %Unlike conformal meshes, NURBS's degrees of freedom do not lie on the surface, thus it's hard to enforce Dirichlet conditions by holding a subset of them fixed. Moreover, the 
%in which basis functions emanating from computer aided geometric design (CAGD) are utilized in finite element analysis as well. 
The proposed method in this study falls in line with isogeometric analysis. But here, 
%use bicubic Hermite patches to describe geometry and model shell dynamics using displacement-only NURBS shell. 
%An underlying premise is that the NURBS geometry, which possesses global smoothness,
%is more suited for describing wrinkles or folds that are the characteristics of cloth motion.
%Since only the mid-surface is adequate for representing and simulating the overall thin volume, potentially we can leverage the parametric surface modelling technology to facilitate better simulation. 
%In this paper, 
%we utilize bicubic Hermite basis as the underlying representation for both geometry and physical field interpolation. 
we develop a unified framework for thin-shell simulation which seamlessly integrates midsurface geometric modeling, dynamics simulation, as well as ray-tracing for rendering, all utilizing bicubic Hermite patches as the underlying representation. 
%Still using the original linear finite element method for parametric thin shells analysis will not only bring cumbersome remodeling burden, but also introduce serious discretization errors.
%Then it's necessary to develop a new numerical solver tailored for parametric surface represented thin shell to fully explore its advantages on smoothness and controlability. 
% Compared with triangular meshes, the parametric surfaces are inherently smoother, more precise, and a great amount of control and flexibility. 
%In order to eliminate this dilemma, we dedicated to developing a comprehensive framework for thin shell simulation which seamlessly integrate parametric geometric modeling, dynamics simulation, and ray-tracing rendering by using unified representation. 

Specifically, we present two main contributions to achieving this goal.
\textbf{First, we devise an implicit Bicubic Hermite finite-element solution for the KL model.}
Bicubic Hermite (BH) patches, as an extension of cubic Hermite curves, are originally invented for freeform surface modelling \cite{Farin2001,Salomon2005}. A BH patch is defined by $16$ parameters ($4$ end points, $8$ tangent vectors at end points, and $4$ twist vectors). 
Since Hermite interpolation precisely passes through the patch function and its first derivative at corners, any surface assembled by BH patches with sharing boundaries is $\mathcal{C}^1$-smooth. 
In our paper, the midsurface of thin shell is constructed in this manner. 
Meanwhile, bicubic Hermite patches are also utilized as computational units in finite element analysis. 
Since the shape function belongs to the Hermite polynomial space, it ensures continuity of deformation-gradient field between elements, such that we can directly derive the discretized form of the hyperelastic energy and integrate it into the governing equations with the help of Gauss--Legendre quadrature.
Provided with energy derivatives, an implicit Euler solver can then be achieved. There is no need to customize discrete approximation forms of any physical quantities. The method, dubbed BHEM (Bicubic Hermite Element Method), can capture smoother and richer geometries with much fewer elements than conventional linear FEMs. This makes our solver highly scalable and efficient, given a shared computational basis for design exploration and optimization.

%High order finite element method for thin shell simulation is not rare in the computational physics field. They usually focus on quasi-static problems, while 
For scenarios with large nonlinear and highly dynamic deformations, there can be rich contacts not only between the shell and its surrounding environment but also among shell sub-parts.
Further consolidating the integration between geometry representation and simulation, and bypass mesh-based collision detection, \textbf{our second main contribution is a BH-surface intersection detection algorithm, which is more intuitive, efficient, and scalable compared with the state-of-the-art methods.} 
Specifically, BH surfaces can be reformulated as the equivalence of B\'{e}zier surfaces. Based on the convex hull property of the B\'{e}zier surface, a bounding-volume-hierarchy (BVH) tree is constructed through dynamic subdivision of the surface and then pruned using Newton's method.
% Specifically, the algorithm subdivides the surface dynamically based on the convex hull property of the B\'{e}zier surface to construct a BVH tree, and prunes it by Newton's method for root finding.
 %On this basis, the intersection of rays and static patches is applied to ray tracing rendering, and the intersection of movable basic geometric elements (such as points, lines, and surfaces) and movable patches is applied to continuous collision detection. 
Thus, taking this as an additional benefit, we can replace the ray-surface intersection modules of a traditional ray tracing method with our BH-surface intersection detection algorithm, resulting in a parametric thin-shell-based ray-tracing.

%Shells are ubiquitous structures found in nature, such as leaves, insect wings, seashells, bubbles and biological membranes. Their visually appealing geometry and desirable mechanical properties have inspired plethora man-made objects design, including cloth, Origami, balloon, architecture, aircraft fuselage and so on. Owing to the wide applications of shell structures, great efforts have been made to the development of advanced theoretical models and numerical methods to accurately and efficiently predict the deflections behaviors of them in the computational physics field. 

%Among these achievements, Kirchhoff-Love(KL) theory is commonly selected for analysing the mechanical behavior of shells with the thickness is small enough compared to the minimal radius of curvature. It assumes that the transverse normals are always remain perpendicular to the midsurface in arbitrary deformed configuration, which implies that there is no transverse shear strains in any shell cross section. 

%Since KL model appealingly reduce the problem of studying deformation of the 3D shell volume to that of deformation of a 2D surface, it gains great attention in computer graphic community for a broad array of thin-shell objects simulation. Our work is based on the  Kirchhoff-Love theory as well. 


%Physics-based simulation of thin shell object, such as cloth~\cite{}, paper(Origami)~\cite{} and skin~\cite{}, is a long-standing focus in computer graphics due to their visually appealing geometry and desirable mechanical properties. 

%The Kirchhoff--Love(KL) theory~\cite{} is widely invoked as the underpinning theoretical model for the thin shell kinematics, which is also the basis of this paper. By assuming the transverse normals are always remain perpendicular to the midsurface throughout the deformation, it can attractively simplify the problem of studying deformation of the 3D shell volume to that of a 2D surface (its midsurface) with a specified thickness, but can yet deal with nonlinear phenomena.  
%Many excellent works~\cite{} have shown that discretizing the Kirchhoff-Love equation with the linear triangular element can produce sufficient accurate result with moderate amount of computational cost. 
%c0 finite element method for Kirchhoff-Love shell simulation can produce sufficient accurate result with moderate amount of computational cost. 

%For numerical implementation, linear triangular elements based on KL model has been proven to be able to produce sufficient accurate results with less computational cost.
%Moreover, the linear triangular elements are selected as the computation unit in the finite element analysis of the KL model, which has been proven to be able to produce sufficient accurate results with less computation cost.

%However, many natural drawbacks of this paradigm have also been recognized.   
%First, the standard linear shape functions of triangular element is too trivial to capture sub-element fine wrinkle structures. Second, the integrability of curvature-based bending energy requires both the displacement field and its first derivative must be smooth in the entire domain. Since linear triangular element can not ensure C1 continuity in the element interface, the bending energy has to be directly discretized in terms of dihedral angles using differential geometry, which implies the shell can only bend along the common edge of adjacent elements. This treatment will leads to severe locking issue, especially when the shell is extremely thin, or the inextensible constraint is enforced. Great efforts have been made to circumvent these locking effects from different aspects, such as using extremely high resolution triangular mesh~\cite{}, runtime remeshing~\cite{}, treating the inextensibility as a hard constraint~\cite{}. 

%In this paper, we dedicate to construct a C1 finite element formalization for KL shell's elastodynamic simulation, which is called Bicubic Hermite Element Method.
%Bicubic Hermite patch, as an extension of Hermite curve, is originally invented for freeform surface modelling~\cite{}. Its shape is defined by 16 parameters (4 end points, 8 tangent vectors at end points, 4 twist vectors). Since Hermite interpolation function precisely passes through the function and its first derivative, any c1 smooth surface can be assembled by a collection of Bicubic Hermite patches with sharing boundaries. 




==> Sections-old/Method.tex <==
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=5cm 2.5cm 5cm 2.5cm,clip,width=0.247\textwidth]{#1}}
    \centering
    \formattedgraphics{Figures/umbrella/umbrella_v001.0015.jpg}
    \formattedgraphics{Figures/umbrella/umbrella_v001.0083.jpg}
    \formattedgraphics{Figures/umbrella/umbrella_v001.0149.jpg}
    \formattedgraphics{Figures/umbrella/umbrella_v001.0219.jpg}
    \caption{The folding process of an oriental paper parasol ($280\times5$ patches), simulated by jointly controlling nodal positions and their first order derivatives. Bending and subtle wrinkles along the ribs can be observed.}
    \label{fig:umbrella}
    \vspace{-0.3cm}
\end{figure*}
\section{The Bicubic Hermite Element Method}
\begin{comment}
Without loss of generality, we assume the parameters $\xi^1,\,\xi^2$ range from 0 to 1, and utilize an orthogonal two-dimensional grid to discretize the parameter space $\omega$. 
A trivial approach to fitting the whole surface is interpolate the sampling points at every nodes of the grid through bi-linear interpolation. However, this breaks the $\mathcal{C}^1$-smoothness on the common edge shared by multiple elements -- the energy turns out to be non-integrable once its density relates to the 2-order partial derivative of the surface. Although Dirac $\delta$ function is commonly used in traditional methods to make it well-defined on the edge, it brings in some drawbacks at the same time: 
casualness when define the relationship between the energy form and the dihedral angle, \emph{locking} phenomenon for bending is only allowed at common edge
, etc. To solve these issues, it's necessary to establish novel approach for surface-fitting through higher-order interpolation methods.
% 上面这段或许更适合放在intro里
\end{comment}
Piecewise bicubic Hermite interpolation can be used to maintain the $\mathcal{C}^1$-smoothness in reconstruction, thus naturally supporting Kirchhoff–Love analysis. This feature motivates us to interpolate both the midsuface geometry and the physical field 
%using the governing equation Eq.~(\ref{eqn:dalembert1}) 
with the same set of bicubic Hermite basis. The numerical recipe for discretization is discussed in this section. 

%The BHEM is applied on the thin-shell midsurface composed of stitched patches (as shown in Fig.~\ref{fig:grid}) to the discretization of the governing equations.
%In this section,
%we aim at solving for the parameterized surface mapping $\bm{x}(\xi^1,\xi^2)$.
%We will give all the numerical recipes containing the geometric representation and quadrature method and discuss how to apply external forces and boundary conditions. 
\begin{figure}[ht]
  \centering
  \begin{tikzpicture}
    \draw[step=0.4] (0,0) grid (2,2);
    \fill (0,0) circle (0.05);
    \fill (0,2) circle (0.05);
    \fill (2,0) circle (0.05);
    \fill (2,2) circle (0.05);
    \node at(-0.2,-0.3) {$(0,0)$};
    \node at(2.2,2.3) {$(1,1)$};
    \node at(-0.2,2.3) {$(0,1)$};
    \node at(2.2,-0.3) {$(1,0)$};
    \draw[ultra thick,color={rgb,255:red,195; green,56; blue,40}] (1.2,0.8) rectangle (1.6,1.2);
    \draw[dashed,color={rgb,255:red,100; green,26; blue,17}] (1.4,0.8) -- (3.8,0.3);
    \draw[dashed,color={rgb,255:red,100; green,26; blue,17}] (1.4,1.2) -- (3.8,1.7);
    %3.5-5.5,线头0.3
    % \draw[step=2] (4.3,0.3) grid (5.7,1.7);
    \draw (3.5,0.3) -- (5.5,0.3);
    \draw (3.5,1.7) -- (5.5,1.7);
    \draw (3.8,0) -- (3.8,2);
    \draw (5.2,0) -- (5.2,2);
    \fill (3.8,0.3) circle (0.05);
    \fill (3.8,1.7) circle (0.05);
    \fill (5.2,0.3) circle (0.05);
    \fill (5.2,1.7) circle (0.05);
    \node at(4.1,0.5) {$\bm{x}_{00}$};
    \node at(4.9,1.5) {$\bm{x}_{11}$};
    \node at(4.1,1.5) {$\bm{x}_{01}$};
    \node at(4.9,0.5) {$\bm{x}_{10}$};
    \node at(5.9,1.7) {$\xi_\mathrm{max}^2$};
    \node at(5.9,0.3) {$\xi_\mathrm{min}^2$};
    \node at(3.8,-0.3) {$\xi_\mathrm{min}^1$};
    \node at(5.2,-0.3) {$\xi_\mathrm{max}^1$};
    \node at(4.5,0.05) {$\Delta\xi^1$};
    \node[rotate=90] at(3.5,1) {$\Delta\xi^2$};
  \end{tikzpicture}
  \caption{Without loss of generality, we assume that the parameters $\xi^1$ and $\xi^2$ range from $0$ to $1$, and utilize an orthogonal two-dimensional grid to discretize the parameter space $\varOmega$. Bicubic Hermite interpolation is conducted within each patch. Naturally, the value of $\bm{x}(\xi^1,\xi^2)$ is determined by the values sampled at the $4$ nearest grid nodes.}
  \label{fig:grid}
\end{figure}

\subsection{Geometric Representation}
As shown in Fig.~\ref{fig:grid}, the geometry of the shell's midsurface is parameterized by stitched bicubic Hemite patches. 
For a single patch, satisfying $\xi^1\in[\xi_\mathrm{min}^1,\xi_\mathrm{max}^1]$ and $\xi^2\in[\xi_\mathrm{min}^2,\xi_\mathrm{max}^2]$, 
any point on its surface can be expressed using its surrounding four nodes' information with bicubic Hermite interpolation as
%is expressed as 
\begin{equation}
  \label{eqn:hermite}
  \bm{x}(\xi^1,\xi^2)=\sum_{p,q,r,s\in\{0,1\}}w_{pq,rs}\left(\frac{\xi^1-\xi_\mathrm{min}^1}{\Delta\xi^1},\frac{\xi^2-\xi_\mathrm{min}^2}{\Delta\xi^2}\right)\bm{x}_{pq,rs}\text{.}
\end{equation}
Here $\bm{x}_{pq,rs}$ represents $4$ generalized coordinates (i.e., the value of the surface mapping, the first partial derivatives, and the second order mixed partial derivative) of node $\bm{x}_{pq}$, with  
%$\bm{x}_{00,rs}$,\,$\bm{x}_{01,rs}$,\,$\bm{x}_{10,rs}$,\,$\bm{x}_{11,rs}$ are the values sampled at the lower-left, lower-right, upper-left, and upper-right nodes respectively, and 
$r$ and $s$ denoting the order of partial derivatives w.r.t. $\xi^1$ and $\xi^2$, respectively.
% \xy{Is this paragraph necessary?}
% The BHEM differs from pure displacement-based interpolation methods in its exploiting of higher-order information, which contribute to the $\mathcal{C}^1$-smoothness on the common edges between discrete patches.
The weight function takes the form of
\begin{equation}
  w_{pq,rs}(\theta^1,\theta^2)=w_{p,r}(\theta^1)\,w_{q,s}(\theta^2)\text{,}
  \label{eqn:hermite_weight}
\end{equation}
where $w_{p,r}$ and $w_{q,s}$are polynomials of at most degree 3,
with $\theta^\alpha\in[0,1]$ defined as $(\xi^\alpha-\xi_\mathrm{min}^\alpha)/\Delta\xi^\alpha$.
We refer readers to \S\ref{apx:hermite} for detailed formulations of bicubic Hermite interpolation.

% \xw{tbd: Hermite interpolation guarantees that (1) the fitted function passes through each sampling point, and (2) in the meanwhile, the derivative of the function takes the same values as the derivatives sampled at each point. 
% These characteristics induce the $\mathcal{C}^1$-smoothness on the common edges between the discrete elements.}

We use the set $\{\bm{q}_I\}$ ($I=1,2,3,\ldots,4N$) to denote all the generalized coordinates of the system with $N$ nodes, each belonging to $\mathbb{R}^3$. Then Eq.~(\ref{eqn:hermite}) over the entire parameter domain is reformulated as
\begin{equation}
  \label{eqn:shape}
  \bm{x}(\xi^1,\xi^2)=\sum_{I=1}^{4N}\varPhi^I(\xi^1,\xi^2)\,\bm{q}_I\text{,}
\end{equation}
in which the \emph{shape functions} $\varPhi^I(\xi^1,\xi^2)$ is derived from the interpolation format of Eq.~(\ref{eqn:hermite}). %\bin{Appendix?}
Since $\varPhi^I$ has compact support, it takes nonzero values only at the 4 nodes of the patch that $(\xi^1,\xi^2)$ lies in, resulting in 16 contributing generalized coordinates.

\subsection{Quadrature Method}
\label{sec:integration}
Taking $\delta\bar{\mathcal{V}}_\mathrm{e}={\partial\bar{\mathcal{V}}_\mathrm{e}}/{\partial\bm{q}_I}\cdot\delta\bm{q}_I$, substituting Eq.~(\ref{eqn:shape}) into Eq.~(\ref{eqn:dalembert1}) yields
{\footnotesize%
\begin{equation}
  \label{eqn:galerkin}
  {\small%
  \sum_{I=1}^{4N}\left(\iint_{\bar{\varOmega}}\left(\varPhi^I\bar{\bm{f}}-\varPhi^I\bar{\rho}h
  \sum_{J=1}^{4N}\varPhi^J\ddot{\bm{q}}_J
  % \ddot{\bm{x}}
  -\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\right)\mathrm{d}\bar{\varOmega}+\int_{\bar{\Gamma}}\varPhi^I\bar{\bm{t}}\,\mathrm{d}\bar{\Gamma}\right)\cdot\delta\bm{q}_I=0}\text{,}
\end{equation}}%
which is a necessary condition of D’Alembert’s principle, indicating that Eq.~(\ref{eqn:dalembert1}) is always true for any virtual deformation interpolated through Eq.~(\ref{eqn:shape}). Due to the arbitrariness of $\delta\bm{q}_I$, every coefficient of $\delta\bm{q}_I$, i.e., the terms in the outermost parentheses, must be equal to zero. Thus, for any $I$ ($1\le I\le 4N$), the following equations hold:
\begin{equation}
  \label{eqn:linear}
  \sum_{J=1}^{4N}M^{IJ}\ddot{\bm{q}}_J=
  \iint_{\bar{\varOmega}}\varPhi^I\bar{\bm{f}}\,\mathrm{d}\bar{\varOmega}+\int_{\bar{\Gamma}}\varPhi^I\bar{\bm{t}}\,\mathrm{d}\bar{\Gamma}-\iint_{\bar{\varOmega}}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\,\mathrm{d}\bar{\varOmega}
  \text{,}
\end{equation}
where each coefficient of the mass matrix is defined as
\begin{equation}
  \label{eqn:mass}
  M^{IJ}=\iint_{\bar{\varOmega}}\bar{\rho}h\varPhi^I\varPhi^J\,\mathrm{d}\bar{\varOmega}=\iint_{\varOmega}\bar{\rho}h\varPhi^I\varPhi^J\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{.}
\end{equation}
Eq.~(\ref{eqn:linear}) is consistent with the result obtained by a Galerkin method that uses shape functions as test functions in the Cauchy equations of motion.
Note here we directly calculate partial derivatives of $\bar{\mathcal{V}}_\mathrm{e}$ with respect to DoFs without introducing deformation gradients.

Due to the compact support of the shape functions $\varPhi$, $M^{IJ}$ is nonzero only when the affected scopes of $\varPhi^I$ and $\varPhi^J$ overlap, in other words, the corresponding generalized coordinates of $\varPhi^I$ and $\varPhi^J$ belong to the nodes of the same patch. Then, for this specific patch, two-dimensional Gauss--Legendre quadrature with 16 points (\S\ref{apx:quadrature}) is adopted for the calculation of nonzero $M^{IJ}$. 
%The compact support of the shape functions implies sparsity of the system -- $M^{IJ}$ is nonzero only when affected scopes of $\varPhi^I$ and $\varPhi^J$ overlap, i.e., the corresponding generalized coordinates of $\varPhi^I$ and $\varPhi^J$ lie in the same patch.
%As for nonzero $M^{IJ}$ and other surface integrals in Eq.~(\ref{eqn:linear}), two-dimensional Gauss--Legendre quadrature with 16 points (\S\ref{apx:quadrature}) is adopted. We traverse first the elements and then the 16 quadrature points in each element to calculate the integrand. An integral is approximated by summation of the integrand values multiplied by corresponding weights.
Note that with $\varPhi^I$ being a polynomial of no more than degree 3, $\varPhi^I\varPhi^J$ reaches a sixth-order at most \update{in each parametric dimension}. The adopted quadrature method provides a seventh-order precision \update{in each parametric dimension}, which enables us to calculate $M^{IJ}$ precisely, given that $\sqrt{\bar{a}}$ is a low-order polynomial with respect to position. %\bin{what's the meaning of the last sentence?}
The surface integral of the internal force in Eq.~(\ref{eqn:linear}) is implemented in the same manner. The treatment of external forces is discussed in the following. 

% The last term of Eq.~(\ref{eqn:linear}) follows the same quadrature form.
%几何用patch，仿真用element
%In order to compute surface integrals in the above equations, we traverse the elements and traverse the quadrature points in each element. The integrals can be approximated by the summation of the sampled values of the integrand at each point multiplied by a corresponding weight.

\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=10cm 0cm 10cm 2.5cm,clip,width=0.163\textwidth]{#1}}
    \centering
    \formattedgraphics{Figures/can/patches_0119.0000.jpg}
    \formattedgraphics{Figures/can/patches_0119.0022.jpg}
    \formattedgraphics{Figures/can/patches_0119.0055.jpg}
    \formattedgraphics{Figures/can/patches_0119.0202.jpg}
    \formattedgraphics{Figures/can/patches_0119.0385.jpg}
        \formattedgraphics{Figures/can/patches_0119.0499.jpg}
    \caption{ A hollow cylindrical shell ($20\times20$ patches) deforms severely under the gradually increased compression. Initially, the cylinder is mounted on the ground; as the wood plank gets pushed down, the deformation of the cylinder manifests locally at first; at some point, the  unshaping takes a sudden change; further compression produces severe deformation and high degree of self contact.
}
    \label{fig:can}
    \vspace{-0.3cm}
\end{figure*}

\subsection{External Forces}
External forces acted on the thin shell usually include areal force and point force. 
%We apply two common categories of external forces on thin shells --- areal forces and point forces. 

We instantiate areal forces as gravity and pressure. Gravity force density is given by $\bar{\bm{f}}_\mathrm{grav}=\bar{\rho}h\bm{g}$ where $\bm{g}$ denotes the gravity acceleration, and pressure force density is given by $\bar{\bm{f}}_\mathrm{press}=p\bm{n}$ with $\bm{n}$ denoting the midsurface normal and $p$ the magnitude of pressure. The integration scheme similar to internal force and mass matrix is applied here to achieve the equivalent forces acting on the generalized coordinates. 
%不太知道这里需不需要说明f和fbar

A point force $\bar{\bm{f}}_\mathrm{pt}$ exerted at arbitrary point $\bm{x}_\mathrm{pt}(\xi^1_\mathrm{pt},\xi^2_\mathrm{pt})$ on the surface can be reformulated as an areal force multiplied by a Dirac $\delta$ function.  %Supposed that a point force $\bar{\bm{f}}_\mathrm{p}$ is applied on an arbitrary point $\bm{x}_\mathrm{p}$ on the surface,
Then, we can directly achieve its closed integral form as 
\begin{equation}
\iint_{\bar{\varOmega}}\varPhi^I\bar{\bm{f}}_\mathrm{pt}\delta(\bm{x}_\mathrm{pt})\,\mathrm{d}\bar{\varOmega}=\sum_I\varPhi^I(\xi^1_\mathrm{pt},\xi^2_\mathrm{pt})\bar{\bm{f}}_\mathrm{pt}\text{.}
\label{eqn:point_force}
\end{equation}
Here, $\varPhi^I(\xi^1_\mathrm{pt},\xi^2_\mathrm{pt})$ indicates the value of the shape function $\varPhi^I$ taken at $\bm{x}_\mathrm{pt}$, which implies that a point force only influences the 16 generalized coordinates of its nearest 4 nodes.

\subsection{Boundary Conditions}
Position constraint (Dirichlet boundary condition) and its derivative constraint (Neumann boundary condition) are handled in our method. 

For specific node, these two constraints can be simply realized by removing their corresponding generalized coordinates from the solution variables and taking their influence back to Eq.~(\ref{eqn:linear}) as a given term. 
%Typically, boundary conditions contain Dirichlet boundary conditions that specify function values and Neumann boundary conditions that specify values of derivatives, both at the domain boundary.
%In our case, the former indicate constraining position values, while the latter indicate constraining position derivatives.
% constrain the directional derivatives of the boundary normal, and a mixture of the two.
% control points: gradient
% 可以直接 
%A trivial way to apply these constraints is to add them on the control points, which is implemented by
%directly freezing the corresponding generalized coordinates. 
Additionally, the position constraint imposed on the element's boundary curve needs to be realized through the combination of the position constraints and the derivative constraint along the boundary tangent direction for every node on the boundary. The boundary's derivative constraint only requires applying appropriate derivative constraint for all going through nodes. 
%a series of constraints applied on every node on the segment. It is proved that the shape of the surface boundary can be completely determined through prescribing the positions and the partial derivatives along the tangent direction at the boundary.
%arbitrary point: augmented Lagrangian method
Furthermore, both types of constraint can be applied at arbitrary points on the midsurface as well. According to \S\ref{apx:hermite}, the position and its derivative at arbitrary points can be represented as a weighted sum of its four surrounding nodes' $16$ generalized coordinates. Thus, the constraints on surface points can be transferred to the constraints on the nodes. However, this conversion is not unique. To circumvent this issue, we can reformulate Eq.~(\ref{eqn:linear}) as a constrained optimization problem if necessary.

%which is then solved by the method of Lagrangian multipliers \cite{}. For more implementation details readers can refer to \S\ref{sec:solver}.
%According to Eq.~\ref{}, the position and its derivative constraint at arbitrary points can be formulated as a weight sum of its four surrounding node's $16$ generalized coordinates, which can be directly integrated into Eq.~(\ref{eqn:linear}).  these formulation with the equation of motion constraint, and sol need to be solved with the equation of motion simultaneously. 

%according to Eq.~\cite{}, for any surface point, no matter for its position and its first order derivative can be represented as a weight sum of its four surrounding nodes'  
% This is achieved by reformulating Eq.~(\ref{eqn:linear}) as a constrained optimization problem, which is then solved by the method of Lagrangian multipliers \cite{}.

Compared with other popular numerical schemes such as the pure displacement-based finite element method and the moving least squares method, the benefits of imposing boundary conditions within our BHEM framework are two folds: 
(1) the present elements turn higher-order derivatives into nodal degrees of freedom, which allows us to precisely control the derivative on every single point on edge, rather than having to fix the two columns of nodes, and yet, to only approximate it;
(2) since the Hermite interpolation precisely passes through the sampled function values and maintains their first-order derivatives, it enables intuitive constraint editing.


%We want to emphasize that the present bicubic Hermite elements  involve higher-order derivatives into the nodal degree of freedoms, and strictly satisfy the  

 %We highlight the convenience to impose boundary conditions within the BHEM framework --- the encoded higher-order information greatly facilitates the intuitive tuning of the thin-shell object.
 
%We emphasize that compared with the pure displacement based finite element method, the present elements involve higher-order derivatives into the nodal degree of freedoms, it allows our method can control the position derivative on single point or edge, rather than fixing two columns of nodes to approximate it. 


%We emphasize that compared with other traditional frameworks, the BHEM exhibits its unique superiority in this regard. 
%For mesh-based methods such as FEM, there is no trivial method to impose a Neumann boundary condition, with the usual practice being fix two rows of nodes at the boundary simultaneously. 
%Moving least squares (MLS) is one of the most commonly used meshless interpolation formats in computer graphics.
% Moving least squares (MLS) and radial basis functions (RBFs) are the two most commonly used meshless interpolation formats in computer graphics. 
%One drawback of MLS is that the control points do not distribute on the interpolated surface, which leads to the fact that simple position constraints cannot be directly added onto control points. Therefore, one has to introduce Lagrangian multipliers to convert the boundary value problem into an optimization problem.
%Our method is similar to RBFs that utilize higher-order information when dealing with boundary value problems.
% On the other hand, although the surface interpolated by RBFs passes through every control point, 
% it gives no way to impose the Neumann boundary condition either.

%compare with RBF: first order
%compare with MLS: directly add on control point

==> Sections-old/Physical-Model.tex <==
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=5cm 2.5cm 5cm 4cm,clip,width=0.247\linewidth]{#1}}
    \centering
    %\formattedgraphics{Figures/needles/needles_v02.0073.jpg}
    %\formattedgraphics{Figures/needles/needles_v02.0086.jpg}
    %\formattedgraphics{Figures/needles/needles_v02.0098.jpg}
    \formattedgraphics{Figures/needles/needles_v02.0126.jpg}
    \formattedgraphics{Figures/needles/needles_v02.0381.jpg}
    \formattedgraphics{Figures/needles/needles_v02.0434.jpg}
    \formattedgraphics{Figures/needles/needles_v02.0498.jpg}
    \caption{A sheet of cloth ($30\times30$ patches) falls on a needle array and then gets pulled away from aside. The bulges on cloth surface are pushed by the needle tips. This sharp geometry deformation caused by the tiny contact demonstrates well the fine resolution of the patch interpolation. }
    \label{fig:needles}
    \vspace{-0.3cm}
\end{figure*}
\section{Continuous Formulations}

As usual, we model the geometry of a 3D thin shell by a 2D curved surface with its uniform thickness as a fixed parameter.
Based upon the Kirchhoff--Love assumption, the continuous formulations of strain, energy, and equations of motion are obtained,
which generally follows the work of \citet{Cirak2000} but is not restricted to linearized kinematics or quasi-static analysis.

\paragraph{Conventions and notations}
For brevity, the Einstein summation convention is followed, where an index variable appears twice in a single term implies summation of that term over all the values of the index.
In the paper, we further assume that the value of an index denoted by a lowercase Latin letter (e.g., $i$, $j$, and $k$) ranges over the set $\{1,2,3\}$, while that denoted by a lowercase Greek letter (e.g., $\alpha$, $\beta$, and $\gamma$) ranges over the set $\{1,2\}$.
Besides,
%covariant and contravariant components of tensors are indicated with lower and upper indices, respectively,
indices appearing after commas imply partial derivatives.

\subsection{Kinematics of Deformation}

We begin by considering a 2D curved surface $\varOmega\subset\mathbb{R}^3$ that is parameterized by curvilinear coordinates $(\xi^1,\xi^2)$. These coordinates form a parameter space $\omega$, where any position vector on the surface is then given by the mapping $\bm{x}:\omega\to\varOmega$. With the basis vectors defined as $\bm{a}_\alpha=\bm{x}_{,\alpha}={\partial\bm{x}}/{\partial\xi^\alpha}$, the unit normal vector on the surface is calculated as $\bm{a}_3={\bm{a}_1\times\bm{a}_2}/{\lVert \bm{a}_1 \times \bm{a}_2 \rVert}$.
According to the Kirchhoff--Love assumption, we can extrude $\varOmega$ by a constant distance $h/2$ in both along and opposite to the surface normal direction $\bm{a}_3$, which forms the volume of a $h$-thick shell. This extrusion is described by a mapping $\bm{r}:\omega^h\to\varOmega^h$ as follows:
\begin{equation}
  \bm{r}(\xi^1,\xi^2,\xi^3)=\bm{x}(\xi^1,\xi^2)+\xi^3\bm{a}_3(\xi^1,\xi^2)\text{,}\quad-\frac{h}{2}\le\xi^3\le+\frac{h}{2}\text{,}
\end{equation}
where $\omega^h=\omega\times[-h/2,+h/2]$ is the extruded parameter space, and $\varOmega^h$ denotes the volume of the extruded shell. In the shell theory, $\varOmega$ is often called the \emph{midsurface}.

To analyze deformation of the extruded shell, we must evaluate the difference between deformed and the undeformed (reference) configurations. These configurations share the same parameter space, $\omega$ and $\omega^h$, but have distinct parametric mappings. For convenience, symbols with overbars are used to indicate quantities in the reference configuration, which suggests the mapping $\bar{\bm{r}}:\omega^h\to\bar{\varOmega}^h$:
\begin{equation}
  \bar{\bm{r}}(\xi^1,\xi^2,\xi^3)=\bar{\bm{x}}(\xi^1,\xi^2) + \xi^3\bar{\bm{a}}_3(\xi^1,\xi^2)\text{,}\quad-\frac{h}{2}\le\xi^3\le+\frac{h}{2}\text{.}
\end{equation}
Here, $\bar{\bm{a}}_3=\bar{\bm{a}}_1\times\bar{\bm{a}}_2/{\lVert\bar{\bm{a}}_1\times\bar{\bm{a}}_2\rVert}$ is the normal vector of $\bar{\varOmega}^h$.

Since the parametric description of the shell is given, we take partial derivatives of $\bm{r}$ and acquire the tangent basis vectors of $\varOmega^h$ as
\begin{subnumcases}{\label{eqn:gdef}\bm{g}_i=\frac{\partial\bm{r}}{\partial\xi^i}=}
  \bm{a}_{\alpha}+\xi^3\bm{a}_{3,\alpha}\text{,}&$i=\alpha<3$,\\
  \bm{a}_3\text{,}&$i=3$.
\end{subnumcases}
Covariant components of the metric tensor are then calculated by dot products as $g_{ij}=\bm{g}_i\cdot\bm{g}_j$, resulting in
\begin{subnumcases}{g_{ij}=}
  a_{\alpha\beta}-2b_{\alpha\beta}\xi^3+c_{\alpha\beta}(\xi^3)^2\text{,}&$i=\alpha<3\land j=\beta<3$,\\
  1\text{,}&$i=j=3$,\\
  0\text{,}&otherwise,
\end{subnumcases}
where
\begin{numcases}{}
  a_{\alpha\beta}=\bm{a}_\alpha\cdot\bm{a}_\beta\text{,}\\
  b_{\alpha\beta}=\bm{a}_{\alpha,\beta}\cdot\bm{a}_3\text{,}\\
  c_{\alpha\beta}=\bm{a}_{3,\alpha}\cdot\bm{a}_{3,\beta}\text{,}
\end{numcases}
correspond to the first, second, and third fundamental forms of the midsurface, respectively.
In a similar way, $\bar{\bm{g}}_i$ and $\bar{g}_{ij}=\bar{\bm{g}}_i\cdot\bar{\bm{g}}_j$ is acquired for $\bar{\varOmega}^h$ as well.

With $\{\bar{\bm{g}}_i\}$ being the basis of the tensor space, the \emph{Green--Lagrange strain} is defined as half the difference between the metric tensors in the deformed and undeformed configurations, i.e.,
\begin{equation}
  E_{ij}=\frac{1}{2}(g_{ij}-\bar{g}_{ij})\text{.}
\end{equation}
As will be readily seen, $E_{ij}$ can be expanded as
\begin{subnumcases}{}
  E_{\alpha\beta} = A_{\alpha\beta}-2B_{\alpha\beta}\xi^3+C_{\alpha\beta}(\xi^3)^2\text{,}\label{eqn:eab}\\
  E_{3\alpha} = E_{\alpha 3} = 0\text{,}\\
  E_{33} = 0\text{,}
\end{subnumcases}
followed by definitions
\begin{numcases}{}
  A_{\alpha\beta}=\frac{1}{2}(a_{\alpha\beta}-\bar{a}_{\alpha\beta})\text{,}\\
  B_{\alpha\beta}=\frac{1}{2}(b_{\alpha\beta}-\bar{b}_{\alpha\beta})\text{,}\\
  C_{\alpha\beta}=\frac{1}{2}(c_{\alpha\beta}-\bar{c}_{\alpha\beta})\text{.}
\end{numcases}
Note that the zeroth-order term $A_{\alpha\beta}$ in Eq.~(\ref{eqn:eab}) represents the \emph{membrane strain}, while the other terms $B_{\alpha\beta}\xi^3+C_{\alpha\beta}(\xi^3)^2$ characterize the \emph{curvature strain}.

\subsection{Governing Equations}

With the kinetic energy and the elastic strain energy denoted as $T$ and $V_\mathrm{e}$, respectively, we analyze dynamics of the shell in the material space by first acquiring the areal energy density as follows:
\begin{gather}
  \bar{\mathcal{T}}=\frac{\mathrm{d}T}{\mathrm{d}\bar{\varOmega}}=\frac{1}{2}\bar{\rho}h(\dot{\bm{x}}\cdot\dot{\bm{x}})\text{,}\\
  \bar{\mathcal{V}}_\mathrm{e}=\frac{\mathrm{d}V_\mathrm{e}}{\mathrm{d}\bar{\varOmega}}=\left(A_{\alpha\beta}A_{\gamma\delta}h+\frac{1}{3}B_{\alpha\beta}B_{\gamma\delta}h^3\right)\bar{H}^{\alpha\beta\gamma\delta}\text{,}
\end{gather}
with $\bar{\rho}$ denoting mass density and $\bar{H}^{\alpha\beta\gamma\delta}$ defined by
\begin{equation}
  \bar{H}^{\alpha\beta\gamma\delta}=\frac{\lambda}{2}\bar{a}^{\alpha\beta}\bar{a}^{\gamma\delta}+\mu\bar{a}^{\beta\gamma}\bar{a}^{\alpha\delta}\text{.}
\end{equation}
Here, $\bar{a}^{\alpha\beta}$ is a contravariant tensor component, which can be calculated by the matrix inversion ${(\bar{a}^{\alpha\beta})}_{2\times2}=(\bar{a}_{\alpha\beta})^{-1}_{2\times2}$.
$\lambda$ and $\mu$, known as the first and the second \emph{Lam\'{e} parameters}, are deduced from Young's modulus $Y$ and Poisson's ratio $\nu$ as $\lambda={Y\nu}/{(1-\nu^2)}$ and $\mu={Y}/{2(1+\nu)}$, respectively.
This formula of $\bar{\mathcal{V}}_\mathrm{e}$ is derived based upon a St.\ Venant--Kirchhoff constitutive model, as suggested by most of the previous studies \cite{Cirak2000, Weischedel2012}.
% Please refer to \S\ref{} for details.

Since the volumetric shell is replaced by its midsurface, we should also reduce any volumetric force that applies on the shell into areal force, by integrating it along the thickness. 
Supposed that the areal density of external force applied on $\bar{\varOmega}$ is $\bar{\bm{f}}$, and the linear density on $\bar{\varGamma}=\partial{\bar{\varOmega}}$ is $\bar{\bm{t}}$, D'Alembert's principle states that for any virtual deformation $\delta\bm{x}$, the following equation holds:
\begin{equation}
  \label{eqn:dalembert1}  \iint_{\bar{\Omega}}\left(\delta\bar{\mathcal{T}}+\delta\bar{\mathcal{V}}_\mathrm{e}\right)\mathrm{d}\bar{\Omega}=\iint_{\bar{\Omega}}\bar{\bm{f}}\cdot\delta\bm{x}\,\mathrm{d}\bar{\Omega}+\int_{\bar{\Gamma}}\bar{\bm{t}}\cdot\delta\bm{x}\,\mathrm{d}\bar{\Gamma}\text{,}
\end{equation}
in which $\delta\bar{\mathcal{T}}=\bar{\rho}h\ddot{\bm{x}}\cdot\delta\bm{x}$ can be interpreted as the virtual work done by the inertia force, and the variation of $\bar{\mathcal{V}}_\mathrm{e}$ is expanded as
\begin{equation}
  \label{eqn:deltave}
  \delta\bar{\mathcal{V}}_\mathrm{e}=\left(h\,\delta a_{\alpha\beta}A_{\gamma\delta}+\frac{1}{3}h^3\,\delta b_{\alpha\beta}B_{\gamma\delta}\right)\bar{H}^{\alpha\beta\gamma\delta}\text{,}
\end{equation}
owing to the exchange symmetry of indices.

It is noteworthy that the surface area element $\mathrm{d}\bar{\varOmega}$ can be expressed in the parameter space by
\begin{gather}
  \mathrm{d}\bar{\varOmega}=\sqrt{\bar{a}}\,\mathrm{d}\xi^1\mathrm{d}\xi^2\text{,}\\
  \bar{a}=(\bar{\bm{a}}_1\times\bar{\bm{a}}_2)^2=\bar{a}_{11}\bar{a}_{22}-\bar{a}_{12}\bar{a}_{21}\text{.}
\end{gather}

==> Sections-old/Related-Work.tex <==
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=5cm 0cm 5cm 0cm,clip,width=0.163\linewidth]{#1}}
    \centering
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0060.jpg}
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0077.jpg}
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0091.jpg}
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0120.jpg}
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0143.jpg}
    \formattedgraphics{Figures/ball/ball_obj_30_v01.0187.jpg}
    \caption{A sheet of square cloth ($30\times30$ patches) drapes on a ball, exhibiting rich wrinkle patterns in the process of reaching a steady state.}
    \label{fig:ball}
\end{figure*}

\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=8cm 0.5cm 8cm 3.5cm,clip,width=0.163\linewidth]{#1}}
    \centering
    \formattedgraphics{Figures/armadillo/armadillo.0067.jpg}
    \formattedgraphics{Figures/armadillo/armadillo.0082.jpg}
    \formattedgraphics{Figures/armadillo/armadillo.0103.jpg}
    \formattedgraphics{Figures/armadillo/armadillo.0140.jpg}
    \formattedgraphics{Figures/armadillo/armadillo.0176.jpg}
    \formattedgraphics{Figures/armadillo/armadillo.0212.jpg}
    % \includegraphics[trim=9cm 0.5cm 7cm 3.5cm,clip,width=0.32\linewidth]{Figures/armadillo/armadillo.0140.jpg}
    % \includegraphics[trim=7cm 0.5cm 9cm 3.5cm,clip,width=0.32\linewidth]{Figures/armadillo/armadillo.0176.jpg}
    % \includegraphics[trim=8cm 0.5cm 8cm 3.5cm,clip,width=0.32\linewidth]{Figures/armadillo/armadillo.0212.jpg}
    \caption{A sheet of square cloth ($30\times30$ patches) drapes on an armadillo model, where the sharp edges of the model are reflected by the cloth deformation.}
    \label{fig:armadillo}
\end{figure*}

\section{Related Work}

\paragraph{Thin-shell simulation}
Physics-based thin shell simulation, such as cloth \cite{Baraff1998, Choi2002, Bridson2003, Tamstorf2015, Guo2018, Chen2021, Wang2021, Zhang2022}, paper (Origami) \cite{Narain2013, Chen2018, Burgoon2006, Pfaff2014} and skin \cite{remillard2013, Li2018}, is a long-standing topic in computer graphics owing to their visually appealing geometry and desirable mechanical properties. 
%The seminal work of Terzopoulos  to the graphics community a continuum shell model
% Continuum models for elastic surfaces
The seminal work \cite{terzopoulos1987} represents the first continuum models for elastic deformable surfaces from a pure geometric view. 
%In his model, the deformation of first, second and fundamental form in differential geometry are used for modeling the bending energy. 
Following this pioneer work, a series of discrete constitutive models \cite{Grinspun2003, Bridson2003, Gingold2004} are developed directly for the elastic strain energy approximation by applying geometric operators over piecewise-linear surface. 
%Their bending energies are functions of dihedral angle. 
Restricted to inextensible shell only, \citet{Bergou2006} argues the bending energy maintains a much simpler quadratic form, which enables fast time-integration of cloth dynamics. 
\citet{Gingold2004} defines discrete bending strain over faces of a triangle mesh, which is more consistent with the corresponding continuum part.
\citet{Quaglino2016} points out that set bending strain (energy) as a function of the dihedral angle implies that the surface can only bend along the edge of mesh, which will lead to severe locking issues especially when the stretching stiffness is much larger than the bending direction. Dynamic remeshing \cite{Narain2012,  Weidner2018, Bender2013} circumvents this issue by aligning the geometry tessellation with the bending direction, while other solutions treat the inextensible as a hard constraint \cite{Chen2019, Jin2017,Tournier2015}.

The Kirchhoff--Love model \cite{Ciarlet2000} is a commonly adopted continuum mechanic model of thin shell object, in which the shearing deformations are neglected, such that the normal always remain perpendicular to the midsurface throughout the deformation. As a consequence, the shape of a volumetric shell can be fully determined by its midsurface. 
The weak form of KL model could be discretized using a standard finite element approach. As second order derivatives of displacements are involved in the bending strain, it requires that the FEM basis functions must be able to reproduce $\mathcal{C}^1$ continuous displacement fields.
%and finding such basis function for unstructured mesh is not trivial. 
Many measures have been taken to circumvent the challenges for finding such basis function for unstructured mesh. As a solution to this problem, some approaches introduce additional variables, e.g. derivatives at edge mid-points \cite{Gingold2004}. 
Non-local interpolation schemes, such as Subdivision FEM, have been used to \cite{Cirak2000, Thomaszewski2006, Clyde2017, Guo2018} circumvent the problem by increasing the support of basis functions over more elements. 
The discontinuous Galerkin (DG) FEM relaxes the restrictive requirement of $\mathcal{C}^1$ continuous basis functions by introducing another deformation energy term which penalizes discontinuities in the derivatives into the governing equation.
Another branch of solution follows the route of isogeometric analysis, in which the basis functions that express geometric shapes is utilized in FEM analysis for the physical fields interpolation \cite{Wawrzinek2011,Lu2014}.
The work of \citet{Qin1994} can be regarded as the first attempt for using NURBS surface to represent the midsurface of a deformable thin object. The global smoothness of the NURBS geometry is exploited \citet{Lu2014} to describe wrinkles or folds that are the characteristics of cloth motion. The shape-matching element method\cite{Trusty2021} utilizes NURBS surface for deformable volumetric object simulation. However, the NURBS representation is complex, the derivation there is more involving and the control is less flexible and intuitive. 

\paragraph{Ray-patch intersection}
The ray-patch intersection is the calculation for finding all or the first intersection points of rays with the surface \cite{Campagna1997}. This is a basic requirement for various operations such as surface modeling, realistic image, CNC tool path planning. Any desirable surface intersection technique has to balance three conflicting goals of accuracy, robustness, and efficiency.

For direct ray-patch intersection method, the line containing the ray is represented as the intersection of two implicit planes. Substituting the parametric representation of the patch into these implicit equations yields  the intersections of the patch with each of the plane, which is a two-variable high order equations. The root of these equations is the parameter coordinates of the intersection points on the surface. Early approaches for solving these equations are based on numeric techniques such as algebraic resultant elimination \cite{Kajiya1982,  Manocha1994}, implicitization \cite{Manocha1991} or Newton iteration \cite{Toth1985, Martin2000, Geimer2005, Benthin2006, Abert2006}. These methods can deliver high quality solutions with small memory consumption, but the computation cost is intolerable, and numerical issues (e.g., initial value, tangential rays) must be carefully treated. 

Geometric algorithms such as adaptive subdivision \cite{Nishita1990, Tejima2015, Whitted1980, Rogers1984, Woodward1989} and various bounding volume hierarchies are usually adopted to reduce the number of intersection tests or provide initial guesses for the Newton Iteration.
Bezier-clipping \cite{Nishita1990, Tejima2015} is a classical subdivision method which leverages the convex hull property of Bezier curves to recursively prune the region of accepted parameter ranges until the ranges converge to points. 
%Subdivision based algorithms ~\cite{Whitted 1980; Rogers 1985; Woodward 1989} 
%use the convex hull property of parametric patches to determine the ray-patch intersection by subdividing a polygonal approximation of the surface up to a given precision. 
Instead of splitting the patch for each ray as Bezier-clipping does, one can also subdivide the entire surface up to a given precision and construct a hierarchy of bounding volumes to boost ray traversal performance. Simple geometric primitives, such as Chebyshev boxing/sphere \cite{Slusallek1995, Barth1993}, Convex hulls \cite{Pabst2006, Martin2000}, axis aligned bounding box \cite{Geimer2005, Abert2006} are the popular choice for the bounding volume representations. 

%\paragraph{Thin shell simulation}
%Mesh based method

%Meshless method

%Hierarchical, EoL
%\paragraph{Locking}
%\paragraph{Intersection}
%Bezire Clipping, mesh method one sentense


==> Sections-old/Results.tex <==
\section{Results}
We design a wide range of validation tests and simulation experiments to evaluate the validity, fidelity, and effectiveness of our framework from various aspects.
All of the experiments are run on 
% a $6$-core $3.2$GHz Intel(R) Core(TM) i7-8700 desktop with $16$ GB RAM.
\update{a $3.50 GHz$ 13th Gen Intel(R) Core(TM) i5-13600KF desktop with $32$ GB RAM.}

\subsection{Validation}
\begin{figure}[t]
    \centering
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=2cm 4cm 2cm 4cm,clip,width=\textwidth]{#1}}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=1.png}
        \caption{$1\times1$ patch;}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=5.png}
        \caption{$5\times5$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=10.png}
        \caption{$10\times10$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=15.png}
        \caption{$15\times15$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=20.png}
        \caption{$20\times20$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
        \centering
        \formattedgraphics{Figures/wrinkle/wrinkle_obj_size=30.png}
        \caption{$30\times30$ patches.}
    \end{subfigure}
    \caption{Wrinkled sheets. Sheets of different resolutions buckle under uniaxial stretching. (a) There appears only one artificial bump on a single patch. (b) No apparent wrinkle on a shell composed of $5\times5$ patches. (c) A $10\times10$-patch sheet manages to produce several shallow wrinkles. (d) Clearer wrinkles are produced by a $15\times15$-patch sheet. (e) Though wrinkles are finer, but the difference is subtle compared with the previous. (f) The wrinkle pattern converges when it is finer than $30\times30$ patches.}
    \label{fig:wrinkle}
    \vspace{-0.3cm}
\end{figure}

\paragraph{Wrinkled sheets.}
We first validate the accuracy and convergence of our BHEM method with a standard stretched sheet experiment, which is firstly proposed by the pioneering work of \citet{Cerda2003} and later used in both physical engineering \cite{WANG2018} and computer graphics \cite{Vouga2022} community as well. In this experiment, a rectangular thin sheet is pulled apart from its two ends. Due to the high Poisson ratio, the sheet compresses in the perpendicular (vertical) and generates horizontal wrinkles. 
%We begin with validating the soundness and expressiveness of our spatial numerical format through a simple but delicate scene of sheets wrinkling under uniaxial stretching.
%A rectangle sheet being pulled apart horizontally at the left and right boundaries will produce several central wrinkles due to the compression in the vertical direction. 
%After the pioneering work of \citet{Cerda2003}, this phenomenon requires has been studied by many in both physical engineering \cite{WANG2018} and computer graphics \cite{Vouga2022}.

We simulate this model problem with the same physical parameter settings as in the work of \cite{Vouga2022}, which are $\SI{0.25}{\meter} \times \SI{0.1}{\meter}$ for size, $\SI{0.1}{\milli\meter}$ for thickness, Poisson ratio  $\nu= 0.5$ and
Young’s modulus $Y=\SI{1}{\mega\pascal}$.
According to the conclusion of \citet{Vouga2022}, the traditional triangular finite-element-based method needs high resolution ups to tens of thousands of vertices to generate correct wrinkle patterns in this example.  
%Recent work by \citet{Vouga2022} utilized various frameworks to simulate such structure and showed that pure FEM using Delaunay mesh achieve relatively accurate effects only at a rather high resolution (tens of thousands of vertices).
%We perform experiments under the same setting as \citet{Vouga2022}. 
As shown in Fig.~\ref{fig:wrinkle}, the BHEM starts to give apparent wrinkles at a resolution of merely $10^2$ patches (1,452 DoFs in total). As the resolution increases over $15^2$, the difference in the shape of wrinkles is already imperceptible. 
%and has visually converged when the resolution is greater than $15^2$, which strongly demonstrates the outstanding capability of our geometric representation.

We further verify this observation through a quantitative experiment which measures the peak amplitude of wrinkles produced with increased resolution. 
According to the physical experiment results reported by \citet{WANG2018}, the sheet is expected to produce wrinkles with a peak amplitude of $\SI{0.35}{\milli\meter}$. 
The curve illustrated in Fig.~\ref{fig:wrinkle_curve} shows that our BHEM can stably yield $\SI{0.34}{\milli\meter}$ peak amplitude when the simulation resolution is greater than $30^2$ patches (11.5k DoFs in total). While the peak amplitude can only reach to $\SI{0.31}{\milli\meter}$ for the traditional FEM simulated on a triangular mesh with 130k vertices (520k DoFs in total).

%The relative error of that obtained by BHEM is reduced to $15\%$ once the number of patches reaches $12^2$, and is further smoothed to a negligible magnitude after $30^2$. Compared with 0.31mm amplitude generated by FEM with 130k vertices, we obtained much more accurate result using much less degrees of freedom --- $30^2$ patches corresponds to a 3.6k-vertex mesh on the scale, yielding peak amplitude of 0.34mm.

\begin{figure}[t]
%textwidth
\centering
\includegraphics[width=\linewidth]{Figures/wrinkle.eps}
\caption{Statistic of the wrinkle's peak value. The simulated amplitude increases with the refinement of the sheet and converges rapidly to a physical real value ($\SI{3.5e-1}{\milli\meter}$). 
%Lively shapes at specific resolutions are illustrated in Fig.~\ref{fig:wrinkle}
}.
\label{fig:wrinkle_curve}
\end{figure}

\begin{figure}[t]
    \centering
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=4.25cm 1.75cm 6cm 3.5cm,clip,width=\textwidth]{#1}}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/drape10_obj.0039.png}
        \caption{$10\times 10$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/drape20_obj.0039.png}
        \caption{$20\times 20$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/drape30_obj.0039.png}
        \caption{$30\times 30$ patches;}
    \end{subfigure}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/mesh500.0039.png}
        \caption{500 vertices;}
    \end{subfigure}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/mesh2k.0039.png}
        \caption{2k vertices;}
    \end{subfigure}
    \begin{subfigure}{0.324\linewidth}
        \centering
        \formattedgraphics{Figures/drape/mesh8k.0039.png}
        \caption{8k vertices.}
    \end{subfigure}
    \caption{Draped cloth. (a)--(c) shows the results simulated under BHEM framework, while (d)--(f) shows the results simulated under FEM framework. It is clear that BHEM attains higher efficiency in spatial representation.}
    \label{fig:drape}
    \vspace{-0.3cm}
\end{figure}

\paragraph{Draped cloth.}
We conduct a comparative experiments to further demonstrate the superiority of our geometric discretization format. In this scenario, a square piece of cloth, clamped on its four corners, drapes from a flatten configuration under the influence of gravity. 
In Fig.~\ref{fig:drape}, we demonstrate the results simulated with our BHEM and standard FEM (\emph{Libshell} \footnote{https://github.com/evouga/libshell}) under different discretization resolutions respectively. The comparison in the first two columns of Fig.~\ref{fig:drape} shows that our method produces more rich and vivid wrinkles when the number of DoFs is comparable (1,452 DoFs for $10^2$-patch BH surface, and 1,500 DoFs for $500$ vertex). When using high discretization resolution (8k vertex with 24k DoFs ), the quality of standard FEM improved obviously, however our method can achieve the similar quality requiring only 11.5k DoFs ($30^2$ BH patches). For the comparison result, please refer to the third column in Fig.~\ref{fig:drape}. 

%using BHEM and FEM implemented by the widely-used open-source library of \emph{Libshell} \cite{}. We pick a specific frame
%of the simulation with different methods and resolutions and display them in Fig.~(\ref{fig:drape}), the top row and the bottom row representing the results utilized by BHEM and FEM respectively. Clearly, our method gives more vivid wrinkles with similar degrees of freedom (1.2k dgrees of freedom with $10^2$-patch BH surface compared to 1.5k with 500-vertex FEM) and similar performance with less degrees of freedom (10.8k dgrees of freedom with $10^2$-patch BH surface compared to 24k with 8k-vertex mesh).
%We thus claim that BHEM contributes higher efficiency in spatial representation.

\begin{figure}[t]
    %\newcommand{\formattedgraphics}[1]{\includegraphics[trim=8.5cm 1cm 8.5cm 1cm,clip,width=0.324\linewidth]{#1}}
    \centering
    %\formattedgraphics{Figures/drill/dirll.0070.jpg}
    %\formattedgraphics{Figures/drill/dirll.0165.jpg}
    %\formattedgraphics{Figures/drill/dirll.0244.jpg}\\
    %\formattedgraphics{Figures/drill/DirllGrid_png.0070.png}
    %\formattedgraphics{Figures/drill/DirllGrid_png.0165.png}
    %\formattedgraphics{Figures/drill/DirllGrid_png.0244.png}\\
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=0cm 0cm 0cm 0cm,clip,width=0.324\linewidth]{#1}}
    \formattedgraphics{Figures/drill/dirll_transparent.0070.png}
    \formattedgraphics{Figures/drill/dirll_transparent.0165.png}
    \formattedgraphics{Figures/drill/dirll_transparent.0292.png}
    \caption{Twisting cloth ($30\times30$ patches). A buckling swirl around the center as the first-order derivatives (indicated by the red arrows) of the center point rotating horizontally with a constant speed.}
    \label{fig:drill}
    \vspace{-0.3cm}
\end{figure}

%In this example, a cloth 
%the two first-order partial derivatives (red arrows shown in Fig.~\ref{fig:drill}) of the cloth center point rotate with a constant speed in the horizontal plane.  a cloth is successfully drilled by controlling its center point's two first-order partial derivatives 
%We then verify in isolation the effectiveness of the generalized coordinates used to encode higher-order information by drilling an initially axis-aligned square piece of cloth composed by $30^2$ patches. 
% The first-order partial derivatives with respect to $\xi^1,\,\xi^2$ are initialized to be horizontal and vertical respectively at each control point. 
%We pin the single control point at the center of the sheet and drill the sheet by rotating the two coordinate vectors of first-order partial derivatives of the center point (indicated by red arrows in Fig.~(\ref{fig:drill})) simultaneously and uniformly. 
%As shown in Fig.~(\ref{fig:drill}), the drilled cloth rendered with cloth material parameters and with grid wireframe are displayed in the top row and the bottom row respectively, each column extracted at a certain moment from the simulation. 
%The drilling of totally $140^{\circ}$ generates fancy swirl around the center, which demonstrates the 


\paragraph{Parametric surface rendering}
Our proposed ray-surface intersection algorithm would be regarded as a substantial enrichment for current off-the-shell ray-tracing rendering engine. By simply substituting the current ray polygon intersection detection module in pbrt-v4\footnote{https://github.com/mmp/pbrt-v4} with our algorithm, pbrt-v4 can realize parametric surface ray-tracing rendering with different visual effects, as shown in the most right columns of Fig.~\ref{fig:teapot} and Fig.~\ref{fig:caustic}. The other columns are the rendering results for the polygon meshes generated from the parametric surface subdivision. From left to right, the subdivision level gradually increase. Parametric surface naturally processes continuous normal vector on its surface. Fairly fine mesh is required to achieve similar rendering result. 
%Parametric surface naturally processes continuous normal vector on its surface, 
%presented in Section~\ref{} provides a fundamental solution for parametric surface ray-tracing rendering. By replaceing the original ray polygon intersection detection modules in PBRT-4 with our al
%by replacing the  We replace the ray polygon intersection detection modules in PBRT-4 with our 
%We compare our representation of our geometry with triangle mesh shown in Fig.~(\ref{fig:teapot}) and Fig.~(\ref{fig:caustic}). 
%We show that direct rendering free-form surface are smoother through the reflection of environment and caustic of glass.
%The triangle mesh can approximate the surface by subdivision.
%The caustics of mesh have fine and complex grain due to the object isn't smooth enough.



%\paragraph{Rendering performance}

%wrinkle, drill, Hessian, render(time performance, effect compared with mesh)

\begin{figure}[t]
\includegraphics[trim = 0cm 0cm 0cm 0cm, clip,width=\linewidth]{Figures/cantilever.eps}
\caption{\update{Our results on 2D cantilever test.}}
\label{fig:cantilever}
\vspace{-0.3cm}
\end{figure}

\begin{figure}[t]
\includegraphics[trim = 0cm 0cm 0cm 0cm, clip,width=\linewidth]{Figures/lateralbuckling.eps}
\caption{\update{Our results on 3D lateral buckling test.}}
\label{fig:lateralbuckling}
\vspace{-0.3cm}
\end{figure}

% \begin{figure}[t]
% \includegraphics[width=0.48\linewidth]{Figures/cantilever.eps}
% \includegraphics[width=0.48\linewidth]{Figures/lateralbuckling.eps}
% \end{figure}

\paragraph{2D cantilever beam and 3D lateral buckling}
\update{We further valid our method by comparing tow experiments with their theoretical solutions purposed by \citet{}. 
The first is cantilever beam experiment. 
We fix one end of a beam and let it bend under gravity. Its master curve uniquely determines the aspect ratio $H/W$ of cantilever beam under equilibrium as a function of the dimensionless parameter $\Gamma^* = 12(1-\nu^2)\rho gL^3/Yh^2$. 
The second is lateral buckling experiment with the plate lies vertically in the $(x,z)$ plane. We let the plate hang and sag under its own weight and wait for a bifurcation to occur. Its master curve determines when the plate buckle in the third direction as $\Gamma^*$ increases under given aspect ratio $w/L$.
We conduct our results using methods and physical parameters provided by \citet{}. The beam in cantilever test is discretized in $1\times 100$ patches. And the plate is discretized in 20 patches per meter. Our results perfectly matches the master curve as shown in ~\ref{fig:cantilever} and ~\ref{fig:lateralbuckling}.}
% We superimpose our results onto theoretical solutions presented in \citet{}. Our results are in excellent agreement with the master curve.

\subsection{Experiments}

\begin{figure}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=5.5cm 2cm 5.75cm 1.5cm,clip,width=0.324\linewidth]{#1}}
    \centering
    \formattedgraphics{Figures/locking/locking_10.0027.jpg}
    \formattedgraphics{Figures/locking/locking_10.0042.jpg}
    \formattedgraphics{Figures/locking/locking_10.0074.jpg}\\
    \formattedgraphics{Figures/locking/locking_10_slide.0001.jpg}
    \formattedgraphics{Figures/locking/locking_10_slide.0057.jpg}
    \formattedgraphics{Figures/locking/locking_10_slide.0098.jpg}
    \caption{A thin sheet ($10\times10$ patches) with its two diagonal ends fixed bends by gravity. After reaching steady state, the fixed points slide smoothly along the opposite edges without any locking artifacts from discretization. We emphasize that only $10\times10$ patches are used here.}
    \label{fig:locking}
    \vspace{-0.3cm}
\end{figure}
\paragraph{Locking}

The BHEM formulation doesn't need any special treatment, such as dynamic remeshing, to avoid the locking issue, even with very few degrees of freedom. 
As shown in the top row of Fig.~\ref{fig:locking}, a squared piece of cloth, which is composed of $10^2$ patches, is initially pinned at its two diagonal corners. As the pinning points slide along the boundary, the cloth can naturally fold down along any direction as illustrated in the bottom row of Fig.~\ref{fig:locking}. 
%We test the typical setting of a square piece of cloth hanged by pinning a pair of diagonal corner nodes to demonstrate that BHEM successfully overcomes the membrane locking issue that traditional numerical formats suffer from. Self-collisions are also handled properly.
%As shown in the top row in Fig.~(\ref{fig:locking}), a $10^2$-patch square sheet of cloth yields qualitatively plausible results. Our interpolation format allows bending along arbitrary direction, which is emphasized by the experiments illustrated in the bottom row. We \emph{continuously sliding} the two pinned points along the opposite boundaries toward opposite directions and the cloth appears no spurious locking phenomenon throughout the simulation, even with a rather coarse background grid.


\paragraph{Twisting cloth.}
Our method allows precise and intuitive control over the first-order derivatives of an arbitrary point on the surface. 
In this example, the center point of a squared piece of cloth is fixed. And its two first-order partial derivatives (indicated by the red arrows in Fig.~\ref{fig:drill} are rotated with a constant speed in the horizontal plane. 
This prescript motion results in a persistent compression perpendicular to the first derivative directions, and eventually invokes the buckling swirl around the center.
%As shown in Fig.\ref{fig:drill}, the cloth uniformly buckled and all the wrinkles swirl around the center in a delicated way.
In a pure displacement-based method, a similar result can only be achieved through prescript at least three nodes' motion. 

\paragraph{Cloth draping on objects.}
%We validate our CCD and collision handling algorithms by cloth pieces falling onto different 
Both resting and dynamic contact can be faithfully detected and resolved within our framework. 
Two square sheets of cloth, both of which are composed of $30^2$ patches, drape on a parametric sphere and a triangular meshed armadillo are demonstrated in Fig.~\ref{fig:ball} and Fig.~\ref{fig:armadillo} respectively. Rich deformation details due to the interference from external objects can be observed in the results. Please see the supplemental video for more visual evidence.
%Contacts in both scenarios are treated properly, including rest contact and continuous contact with tangential sliding. Please see the supplemental video for more visual evidence.

%As shown in Fig.~(\ref{fig:ball}), the cloth with its two corners fixed drapes on a sphere represented by implicit function. 
%hangs on its left boundary and generates a bump after caught in collision with a sphere described by implicit representation.
%Another example is shown in Fig.~(\ref{fig:armadillo}), where the cloth falls to cover the armadillo with triangulated mesh from above, with folds and wrinkles horned by its protrusions clearly displayed.
%Contact in both scenarios get proper treatment, including rest contact and continuous contact with tangential sliding. Please see the supplemental video for more visual evidence.

\paragraph{Cloth sliding over needles.}
% geometric (smoothly sliding) collision (robust with no )
%The HBEM formulation can capture smoother and richer geometries with much fewer finite elements. 

In this example, we drop a sheet of cloth on a needle array, and then pull it away from aside. The subtle bulges on cloth surface, which are pushed out by the needle tips, can be clearly observed in Fig.~\ref{fig:needles}. 
In the supplemental video, we can easily notice that when pulling the cloth over the needle array, the cloth exhibits natural choppy movement around the needle tips due to the contact interaction. 
These two points verify that our BHEM formulation and collision detection algorithm can handle sharp geometry features robustly.
 
%We examine the performance of BHEM with sharp features by a $30^2$-patch square sheet falling onto needles stuck on a board. Subtle bulges prodded by needle tips can be clearly seen from Fig.~(\ref{fig:needles}) and the cloth is able to steadily rest on the tips without observable jitters.
%When we drag it by the two corner nodes on the right boundary, the cloth managed to \emph{slide smoothly} upon the needles tips without getting stuck or jolted, and produce plausible traces of continuous sliding.

\paragraph{Folding an oriental paper parasol. }
%We further validating our framework by generating buckling patterns under external forces. In the example of Chinese oil-paper umbrella, we begin with an umbrella that is fully put up (the cover forming the side face of a frustum of a cone) and close it under application of gravity and vertical pressure inducing its buckling trend. We imitate an umbrella rib by freezing and appointing values manually to the positions and partial derivatives along the ribs.
%As displayed in Fig.~(\ref{fig:umbrella}), our method generates steady buckling that is in line with physical intuition between each pair of neighboring ribs.
By jointly controlling node positions and their first order derivatives, we can mimic the folding process of an oriental paper parasol driven by the motion of its rib as displayed in Fig.~\ref{fig:umbrella}.


\begin{figure}[t]
    \newcommand{\formattedgraphics}[2]{\begin{subfigure}{0.324\linewidth}\centering\includegraphics[trim=11cm 0cm 11cm 2.5cm,clip,width=\textwidth]{#1}\caption{#2}\vspace{-0.3cm}\end{subfigure}}
    \centering
    \formattedgraphics{Figures/can/can_05mm.0250.jpg}{$h=0.5$mm}
    \formattedgraphics{Figures/can/can_1mm.0250.jpg}{$h=1$mm}
    \formattedgraphics{Figures/can/can_2mm.0250.jpg}{$h=2$mm}
    \caption{ Hollow cylindrical shells ($30\times30$ patches) with different thickness buckles under the gradually increased axial compression. Inside each shell, there is a rigid cylindrical mandrel. Its radius differs from that of the shell by $10\%$. As the wood plank gets pushed down, local buckles can no longer grow unrestrained because their radial displacements are arrested by the mandrel. Thereby, more buckles form and eventually accumulate into a diamond like pattern over the entire surface.}
    \label{fig:cancomp}
    \vspace{-0.3cm}
\end{figure}

\paragraph{Cylindrical shell buckling.}
%BHEM also works well in the set of experiments performed under pure axial compression. We model the cans by cylinders of different thickness, and make it crumple under gradual increase in compression.
In Fig.~\ref{fig:can}, a hollow cylindrical shell severely buckles under the gradually increased compression is simulated with our method.  
When there is an inner mandrel, local buckles can no longer grow unrestrained because their radial displacements are arrested by the mandrel. Thereby, more buckles form and  eventually accumulate into a diamond like pattern over the entire cylinder as shown in Fig.~\ref{fig:cancomp}. The results are consistent with real world experiments~\cite{Seffen2014}.

\begin{table*}[t]
  \centering
  \caption{Here we list the parameters and the time consumed in each example, including 
  \update{the degrees of freedom, the total number of nonzero elements in the BHEM system matrix, }
  the total number of sampling points on the external collider, 
  the properties of the cloth (Young's Modulus $Y\,[\text{Pa}]$, Poisson's ratio $\nu$ and thickness $h\,[\text{mm}]$, mass density $\rho\,[\text{kg}/\text{m}^3]$), 
  Rayleigh damping coefficient $\alpha$, 
  time step $\Delta t\,[\text{ms}]$,
  time consumed in one integration step $t_\mathrm{int}\,[\text{s}]$, in one CCD step $t_\mathrm{obj}\,[\text{s}]$, and whether we detect self-collision (SC, '--' means that CCD has not been performed in this example).}
  \label{tab:experiments}
  \begin{threeparttable}
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c}
      \hline
      Figure& Example& \#\update{DoFs} & \#\update{NNZs} & \#Samples 
      & $Y$ & $\nu$ & $h$ & $\rho$ 
      & $\alpha$ & $\Delta t$ 
      & $t_\mathrm{int}$ & $t_\mathrm{obj}$ & SC\\
      \hline
      \ref{fig:wrinkle}& Wrinkled & -- & -- & -- & $1\times10^6$ & $0.5$ & $0.1$ & $0.93\times10^{3}$ & -- & -- & \update{$63.0$}\tnote{\dag} & -- & --\\
      \ref{fig:drape}& Draped  & --& -- & -- & $1\times10^5$ & $0.3$ & $1$ & $0.93\times10^{3}$ & $0$ & $10$ & \update{$6.01$}\tnote{\dag} & -- & --\\
      \ref{fig:drill}& Twisting & $1.15\times10^4$ & $1.19\times10^6$ & -- & $1\times10^4$ & $0.3$ & $1$ & $0.2\times10^{3}$ & $50$ & $2$ & \update{$0.20$} & -- & --\\
      % \ref{fig:teapot}& Teapot &  & &  &  &  & & & -- & -- & -- & --\\
      % \ref{fig:caustic}& Caustic &  & &  &  &  & & & -- & -- & -- & --\\
      % \ref{fig:performance}& Cylinders &  & &  &  &  & & & -- & -- & -- & --\\
      \ref{fig:locking}& Locking & -- & -- & -- & $1\times10^4$ & $0.3$ & $1$ & $0.2\times10^{3}$ & $2$ & $2$ & \update{$3.38$}\tnote{\ddag} & \update{$4.37$} & yes\\
      \ref{fig:ball}& Ball & $1.15\times10^4$ & $1.17\times10^6$ & -- & $1\times10^5$ & $0.3$ & $0.1$ & $0.2\times10^{3}$ & $2.5$ & $2$ & \update{$4.80$} & \update{$0.0023$} & no\\
      \ref{fig:armadillo}& Armadillo  & $1.15\times10^4$ & $1.19\times10^6$ & $2.8$k & $8.21\times10^5$ & $0.243$ & $0.32$ & $472.6$ & $2.5$ & $1$ & \update{$2.90$} & \update{$1.84$} & no\\
      \ref{fig:needles}& Needles  & $1.15\times10^4$ & $1.19\times10^6$ & $3.6$k & $1\times10^4$ & $0.3$ & $0.1$ & $0.2\times10^{3}$ & $5$ & $2$ & \update{$5.05$} & \update{$26.66$} & yes\\
      \ref{fig:umbrella}& Umbrella & $2.02\times10^4$ & $1.76\times10^6$ & -- & $1\times10^6$ & $0.5$ & $0.1$ & $0.93\times10^{3}$ & $5$ & $2$ & \update{$12.47$} & -- & --\\
      \ref{fig:can}& Can (no mandrel) & $5.3\times10^3$ & $4.97\times10^5$ & -- & $1\times10^8$ & $0.3$ & $2$ & $2.7\times10^{3}$ & $5$ & $2$ & \update{$4.55$} & -- & --\\
      \ref{fig:cancomp}& Cans (with mandrel)  & $1.15\times10^4$ & $1.13\times10^6$ & -- & $1\times10^9$ & $0.47$ & 
      -- & $1.4\times10^{3}$ & $5$ & $0.04$ & \update{$5.29$}\tnote{$\ast$} & \update{$0.0024$} & no\\
      \hline
    \end{tabular}
    \begin{tablenotes}
      \footnotesize
      \item[\dag] The given value is obtained by a $30\times30$-patch shell.
      \item[\ddag] The given value is obtained by a $20\times20$-patch shell.
      \item[$\ast$] The given value is obtained by a $\SI{1}{\milli\meter}$-thick shell.
    \end{tablenotes}
  \end{threeparttable}
\end{table*}


==> Sections/Introduction-backup.tex <==
\section{Introduction}
% Thin-shell structures have significant applications in various fields and have been extensively studied in computer graphics and engineering analysis.
The mechanical behaviors of thin-shell structures are commonly characterized by Kirchhoff--Love (KL) theory \cite{Ciarlet2000} which assumes negligible transverse shear and describes the shell kinetics  by \emph{midsurface}'s in-plane stretching and lateral bending. 
Under this assumption, the energy density function derived from elastic strain involves second order derivatives of displacements (Section~\ref{sec:theory}), thus requiring the $H^2$-regularity of the geometric representation of the midsurface. It implies a $C^1$-continuous surface except for finite number of points, so that the elastic energy is well-defined.
% everywhere on the surface

% 是否添加：linearFEM定义operator的方式意味着弯曲只能在边上，导致locking
% However, today’s overwhelmingly popular choice, i.e., finite element method (FEM), adopts linear interpolation within triangle elements to reconstruct the midsurface. 
However, in today’s overwhelmingly popular choice of linear FEM, its discretized edge-based curvature fails to converge
% Its widely used edge-based curvature failing to converge pointwise 
to the shape operator on element interfaces, regardless of triangulation~\cite{Gingold2004}.
A viable strategy
% that enables midsurface interpolation functions in FEM 
to satisfy such high regularity is to leverage subdivision methods~\cite{Cirak2000,Guo2018,Clyde2017} in mesh generation or refinement. 
% But the resulting basis functions obtained with subdivision methods are generally non-polynomial and non-interpolating \xw{???}, which 
But it complicates both numerical integration and collision handling, as latter needed. 

Isogeometric Analysis (IGA)~\cite{Hughes2005, Cottrell2009} is an appealing alternative to attaining high-order continuous solution space. It utilizes various basis functions emanating from computer aided geometric design (CAGD), such as B-splines~\cite{Hollig2012} and NURBS~\cite{Qin1997, Lu2014, Trusty2021} for accurate and effective geometric representations.
% This category of interpolation formats provides more effective geometric representations for wrinkles and folds nature of thin-shell objects with less degrees of freedom. 
However, as the mainstream of graphics adopts NURBS to represent the surface, one has to apply additional constriants around boundaries~\cite{Lu2014} to obtain the global smoothness of a multi-patch model, which may lead to numerical issues. In fact, this observation is always true for pure displacement-based high-order method with locally-supported basis functions, including subdivision FEM~\cite{Clyde2017}. 

Hermite elements are a special family of IGA basis. They stand out for their inherent guarantee of $C^1$-continuity among patches by containing shared derivatives as degrees of freedom. This sort of elements has been well developed (and found to be beneficial) in solving Kirchhoff plate problems~\cite{Phusakulkajorn2013, GRECO2021113476, GRECO2019, Zienkiewicz2005}. 
A simplest and most widely-used formulation of Hermite patch is the bicubic Hermite interpolation conducted in rectangular elements~\cite{Bogner1965, Petera1994, Beheshti2018}.
% share common issues with nurbs
However, it falls short in geometric flexibility when singular points exist. 
% where less or more than 4 patch corners join together remain untreated. 
Unfortunately, these are common cases in computer graphics because any surfaces that is not homeomorphous to a 2d plane would inevitably produce singularities whose derivatives are not well-defined and thus break the $C^1$-continuity.
% A simplest case is the polar singularity of a sphere, which is inevitable when meshing.
% \cite{BHOLE2022} 
%add: time integration and hessian
Moreover, things always become troublesome when it comes to collision handling and rendering. A common solution in existing studies is triangulate the surface~\cite{Panozzo2023}, which significantly diminishes the value of high-order methods. Other studies try to directly solve these intersection detection problem on high-order surfaces~\cite{Abert2006, Martin2000} using numerical methods, but only provide local minimums. 
% All these defects greatly limit the application of Hermite element method in graphics.

In this work, we are committed to improving above discussed shortcomings and equipping Hermitian elements with graphics-friendly features.
We propose the first complete framework that seamlessly integrates thin-shell elastodynamic simulation, collision handling, and high-fidelity rendering, all utilizing our rectified bicubic Hermite patches as the unified underlying geometric representation.

% Our method is based on traditional Bogner-Forx-Schmit rectangle Hermite elements~\cite{Bogner1965}. We generalize quadrilaterally-meshed Hermite surfaces to cover the singularities where the elements degenerate and traditional Hermite representation comes into difficulties.
First, we delicately design auxiliary degrees of freedom and data structures for patching the singular points where the elements degenerate and traditional Hermite representation comes into difficulties. Our method, dubbed BHEM (Bicubic Hermite Element Method), can handle any globally parameterized surfaces with finite singularities and capture smoother and richer geometries with much fewer elements than conventional linear FEMs. This makes our solution highly scalable and efficient, given a shared computational basis for design exploration and optimization.
%modify: c1-continuity of sigularity

Second, provided with newly proposed Hermite representation, we derive the weak form of the constitutive equations of Kirchhoff-Love thin shells and obtain corresponding governing equations. Then we derive the discretized form of the hyperelastic energy, and its first-order derivative and second-order Hessian matrix, which enables an implicit Euler solver.
% This process is equivalent to that of traditional Hermite method when regularities do not exist, but otherwise gets tougher due to the additional DoFs brought by singularities. 
To simplify the implementation and to accelerate the convergence of the system, we use a combined method of coordinate descent and Newton descent in our numerical solver.
% ~\cite{}\xw{citePD?}. 
% This equiped solver helps to establish a highly scalable and efficient simulation framework on the base of our proposed BHEM.

Last but not least, we proposed a BH-surface intersection detection paradigm that guarantees the find of global minimum, and hence facilitates both CCD and rendering tasks.
% Drawing inspiration from the direct rendering of parametric surfaces, we introduce a novel subdivision-based algorithm utilizing the convex hull property of BHE (as a Bezier surface). 
% It guarantees the find of global minimum, which is always important but tricky in simulation of high-order surfaces. 
We develop a dynamic culling technique, supported by inequality tools, and introduce heuristic pruning based on Newton iterations to enhance efficiency.
% without compromising robustness. 
Our method can be easily migrated into other spline-based surfaces like NURBS patches.
% , since they possess the same core properties.
We believe that this represents an critical missing piece of researches of IGA and will pave the way for new developments.

==> Sections/Method-backup.tex <==
\begin{figure}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=5cm 2.5cm 5cm 2.5cm,clip,width=0.23\textwidth]{#1}}
    \centering
    % \formattedgraphics{Figures/umbrella/umbrella_v001.0015.jpg}
    \formattedgraphics{Figures/umbrella/umbrella_v001.0083.jpg}
    \formattedgraphics{Figures/umbrella/umbrella_v001.0149.jpg}
    % \formattedgraphics{Figures/umbrella/umbrella_v001.0219.jpg}
    \caption{The folding process of an oriental paper parasol ($280\times5$ patches), simulated by jointly controlling nodal positions and their first order derivatives. Bending and subtle wrinkles along the ribs can be observed.}
    \label{fig:umbrella}
    \vspace{-0.3cm}
\end{figure}

\section{The Bicubic Hermite Element Method}

\subsection{Geometric Discretization}

To numerically analyze the statics and dynamics of a thin shell, we divide its midsurface into a collection of bicubic Hermite patches that share information via nodes.
We will first describe how to discretize using only regular (non-degenerate) patches, followed by the introduction of degenerate ones.

\begin{figure}
\centering
\begin{subfigure}{0.495\linewidth}
\centering
\begin{asy}
    size(100);
    defaultpen(fontsize(10pt));
    import graph3;
    
    pen xarcPen=deepblue+0.5bp;
    pen yarcPen=brown+0.5bp;
    
    currentprojection=perspective(3,3,2);
    
    surface s=surface(patch(new triple[][] {
      {(0,0,0),(1,0,0),(1,0,0),(2,0,0)},
        {(0,1,0),(1,0,1),(1,0,1),(2,1,0)},
          {(0,1,0),(1,0,-1),(1,0,-1),(2,1,0)},
            {(0,2,0),(1,2,0),(1,2,0),(2,2,0)}}));
    
    draw(s,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));

    draw(s.s[0].uequals(0)  ,xarcPen);
    draw(s.s[0].uequals(1/3),xarcPen);
    draw(s.s[0].uequals(2/3),xarcPen);
    draw(s.s[0].uequals(1)  ,xarcPen);
    draw(s.s[0].vequals(0)  ,yarcPen);
    draw(s.s[0].vequals(1/3),yarcPen);
    draw(s.s[0].vequals(2/3),yarcPen);
    draw(s.s[0].vequals(1)  ,yarcPen);
\end{asy}
\end{subfigure}
\begin{subfigure}{0.495\linewidth}
\centering
\begin{tikzpicture}
% \draw [help lines] (0,-2) grid (7,2);

% \shade[left color=gray!10,right color=gray!80] 
%   (0,0) to[out=-10,in=150] (2,-2/3) to[out=20,in=-150] (4,1/3) to[out=150,in=-10] (5.5/3,3.7/3) to[out=-150,in=20] cycle;
% \draw (0,0) to[out=-10,in=150] coordinate[pos=0.33](A) coordinate[pos=0.67](B) (2,-2/3);
% \draw (2,-2/3) to[out=20,in=-150] coordinate[pos=0.33](C) coordinate[pos=0.67](D) (4,1/3);
% \draw (4,1/3) to[out=150,in=-10] coordinate[pos=0.33](E) coordinate[pos=0.67](F) (5.5/3,3.7/3);
% \draw (5.5/3,3.7/3) to[out=-150,in=20] coordinate[pos=0.33](G) coordinate[pos=0.67](H) (0,0);

% \draw[name path=curveAF] (A) to[out=20,in=-150] (F);
% \draw[name path=curveBE] (B) to[out=20,in=-150] (E);
% \draw[name path=curveHC] (H) to[out=-10,in=150] (C);
% \draw[name path=curveGD] (G) to[out=-10,in=150] (D);

% \fill [name intersections={of=curveAF and curveHC, by={x}}] (x) circle (0.05);
% \fill [name intersections={of=curveAF and curveGD, by={y}}] (y) circle (0.05);
% \fill [name intersections={of=curveBE and curveHC, by={z}}] (z) circle (0.05);
% \fill [name intersections={of=curveBE and curveGD, by={w}}] (w) circle (0.05);

\draw (4.5,-0.4) -- (6.5,-0.4);
\draw (4.5,1) -- (6.5,1);
\draw (4.8,-0.7) -- (4.8,1.3);
\draw (6.2,-0.7) -- (6.2,1.3);
\fill (4.8,-0.4) circle (0.05);
\fill (4.8,1) circle (0.05);
\fill (6.2,-0.4) circle (0.05);
\fill (6.2,1) circle (0.05);
\node at(5.1,-0.2) {$\bm{x}_{00}$};
\node at(5.9,0.8) {$\bm{x}_{11}$};
\node at(5.1,0.8) {$\bm{x}_{01}$};
\node at(5.9,-0.2) {$\bm{x}_{10}$};
\node at(6.9,1) {$\xi_\mathrm{max}^2$};
\node at(6.9,-0.4) {$\xi_\mathrm{min}^2$};
\node at(4.8,-1) {$\xi_\mathrm{min}^1$};
\node at(6.2,-1) {$\xi_\mathrm{max}^1$};
\node at(5.5,-0.65) {$\Delta\xi^1$};
\node[rotate=90] at(4.5,0.3) {$\Delta\xi^2$};
\end{tikzpicture}
\end{subfigure}
\caption{Caption}
\label{fig:regular}
\end{figure}

\begin{figure}
  \centering
  \begin{subfigure}{0.495\linewidth}
    \centering
    \begin{asy}
    size(100);
    defaultpen(fontsize(10pt));
    import graph3;
    
    pen xarcPen=deepblue+0.5bp;
    pen yarcPen=brown+0.5bp;
    
    currentprojection=perspective(3,3,2);
    
    int m=8;
    int n=16;
    real R=2;
    real a=0.6;
    
    triple fs(pair t) {
    return (R*t.x,a*Cos(t.y),a*Sin(t.y));
    };
    
    pair p,q;
    
    for(int i=0;i<n;++i){
    for(int j=0;j<m;++j){
      p=(j/m,i*360/n);
      q=((j+1)/m,i*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen);
      q=(j/m,(i+1)*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen);
    }
    };
    for(int i=0;i<n;++i){
      p=(1,i*360/n);
      q=(1,(i+1)*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen);
    }
    
    surface s=surface(fs,(0,0),(1,360),1,32,Spline);
    //draw(s,surfacepen=material(lightyellow+opacity(.9), emissivepen=0.2*white),render(compression=Low,merge=true));
    draw(s,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));

    p=((m-1)/m,0*360/n);
    q=((m-2)/m,0*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen,Arrow3
    //(TeXHead2(normal=Y))
    //,L=Label("$u$",position=EndPoint,align=N)
    );
    
    p=(m/m,1*360/n);
    q=(m/m,(1+1)*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3
    //(TeXHead2)
    //,L=Label("$v$",position=EndPoint,align=N+E)
    );
    \end{asy}
    \caption{caption}
    \label{fig:cylinder}
  \end{subfigure}
  \begin{subfigure}{0.495\linewidth}
    \centering
    \begin{asy}
    size(100);
    defaultpen(fontsize(10pt));
    import graph3;
    
    pen xarcPen=deepblue+0.5bp;
    pen yarcPen=brown+0.5bp;
    
    currentprojection=perspective(5,4,6);
    
    int m=16;
    int n=8;
    real R=2;
    real a=1;
    
    triple fs(pair t) {
    return ((R+a*Cos(t.y))*Cos(t.x),(R+a*Cos(t.y))*Sin(t.x),a*Sin(t.y));
    };
    
    pair p,q,v;
    
    for(int i=0;i<n;++i){
    for(int j=0;j<m;++j){
      p=(j*360/m,i*360/n);
      q=((j+1)*360/m,i*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen);
      q=(j*360/m,(i+1)*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen);
    }
    };
    
    surface s=surface(fs,(0,0),(360,360),10,10,Spline);
    draw(s,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));

    p=(0*360/m,1*360/n);
    q=((0+1)*360/m,1*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen,Arrow3
    //,L=Label("$u$",position=MidPoint,align=S)
    );
    
    p=(0,1*360/n);
    q=(0,(1+1)*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3
    //,L=Label("$v$",position=MidPoint,align=N)
    );
    \end{asy}
    \caption{caption}
    \label{fig:torus}
  \end{subfigure}
  \caption{Caption}
\end{figure}

\begin{figure}
  \begin{subfigure}{0.495\linewidth}
    \centering
    \begin{asy}
    size(100);
    defaultpen(fontsize(10pt));
    import graph3;
    
    pen xarcPen=deepblue+0.5bp;
    pen yarcPen=brown+0.5bp;
    
    currentprojection=perspective(5,4,6);
    
    int m=10;
    int n=12;
    real R=1;
    
    triple fs(pair t) {
    return (R*Sin(t.x)*Cos(t.y),R*Sin(t.x)*Sin(t.y),R*Cos(t.x));
    };
    
    pair p,q;
    
    for(int i=0;i<n;++i){
    for(int j=0;j<m;++j){
      p=(j*180/m,i*360/n);
      q=((j+1)*180/m,i*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen);
      q=(j*180/m,(i+1)*360/n);
      draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen);
    }
    };
    surface s1=surface(fs,(180/m,0),(180,360),30,30,Spline);
    draw(s1,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));
    
    surface s2=surface(fs,(0,2*360/n),(180/m,360),30,30,Spline);
    draw(s2,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));
    //draw(shift((0,0,1))*scale(0.03,0.03,0.03)*unitsphere, opacity(0.9)+black,currentlight);

    surface s=surface(fs,(0,0),(180/m,2*360/n),10,5,Spline);
    draw(s,surfacepen=material(diffusepen=gray,emissivepen=black, specularpen=black));
    
    p=((3)*180/m,0*360/n);
    q=((3+1)*180/m,0*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),xarcPen,Arrow3
    //,L=Label("$u$",position=EndPoint,align=W)
    );
    
    p=(3*180/m,0*360/n);
    q=(3*180/m,(0+1)*360/n);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3
    //,L=Label("$v$",position=EndPoint,align=N)
    );
    \end{asy}
    \caption{caption}
    \label{fig:degenerate}
  \end{subfigure}
  \begin{subfigure}{0.495\linewidth}
  \centering
  \begin{tikzpicture}[>=latex]
    \def\R{2.25}
    \def\r{0.5}
    \def\l{2.5}
    \node[below left] (O) at (0,0) {$O$};
    \draw (0:\r) -- (0 * 180 / 3:\l);
    \draw (1 * 180 / 3:\r) -- (1 * 180 / 3:\l);
    \draw (2 * 180 / 3:\r) -- (2 * 180 / 3:\l);
    \draw[dashed] (0,0) -- (3 * 180 / 3:0.2);
    \draw[dashed] (0,0) -- (4 * 180 / 3:0.2);
    \draw[dashed] (0,0) -- (5 * 180 / 3:0.2);
    % Concentric arcs
    \draw (-10:\r) arc[radius=\r, start angle=-10, end angle=130];
    \draw (-10:\R) arc[radius=\R, start angle=-10, end angle=130];
    
    \draw[->,draw=red,thick] (0:\R) arc[radius=\R, start angle=0, end angle=45];
    \node at (\R+0.2,0.5) {$\varphi$};
    \draw[->,draw=blue,thick] (0:\r) -- (0:\R);
    \node at (\R-0.5,-0.2) {$r$};
    % \draw[->] (0:0.5) arc[radius=0.5, start angle=0, end angle=60];
    % \node at (0.6,0.4) {$\varphi$};
    % \draw[->] (0,0) -- (0, 1.5);
    % \node at (1.5,0.2) {$\bm{e_1}$};
    % \draw[->] (0,0) -- (1.5, 0);
    % \node at (0.2,1.5) {$\bm{e_2}$};
    \draw [|-|] (0,-0.2) -- node[below=1mm] {\small{$\varepsilon_\mathrm{r}$}} (\r,-0.2);
    %points
    \draw[fill = blue] (\r,0) circle (0.05);
    \draw[fill = blue] (\R,0) circle (0.05);
    \draw[fill = blue] (60:\r) circle (0.05);
    \draw[fill = blue] (60:\R) circle (0.05);
    \draw[fill = blue] (120:\r) circle (0.05);
    \draw[fill = blue] (120:\R) circle (0.05);
    \draw[fill = red] (0,0) circle (0.05);
    \draw[dashed] (\r,0) -- (0,0);
    \node at (\r+0.2,0.2) {\small{$A$}};
    \draw[dashed] (60:\r) -- (0,0);
    \node at (70:\r+0.2) {\small{$B$}};
    \draw[dashed] (120:\r) -- (0,0);
    \node at (110:\r+0.2) {\small{$C$}};
    %partial
    % \draw[->] (\r,0) -- (\r+0.5,0);
    % \draw[->] (60:\r) -- (60:\r+0.5);
    % \draw[->] (\r+0.5,0) -- (\r+0.5,0.5);
    % \draw[->] (60:\r+0.5) -- ({(\r+0.5)*cos(60)-0.5*cos(30)},{(\r+0.5)*sin(60)+0.5*sin(30)});
  \end{tikzpicture}
  \caption{caption}
  \label{fig:polar}
\end{subfigure}
  \caption{Caption}
\end{figure}

\begin{figure}
    \centering
    \begin{asy}
    size(100);
    defaultpen(fontsize(10pt));
    import graph3;
    
    pen xarcPen=deepblue+0.5bp;
    pen yarcPen=brown+0.5bp;
    
    currentprojection=perspective(5,4,6);
    
    int m=10;
    int n=12;
    real R=1;
    
    triple fs(pair t) {
    return (R*Sin(t.x)*Cos(t.y),R*Sin(t.x)*Sin(t.y),R*Cos(t.x));
    };
    
    pair p,q;
    
    surface s1=surface(fs,(0,-30),(72,30),30,30,Spline);
    draw(s1,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));
    
    surface s2=surface(fs,(0,60),(72,120),30,30,Spline);
    draw(s2,surfacepen=material(RGB(190,184,220)+opacity(.9), emissivepen=0.15*white),render(compression=Low,merge=true));
    //draw(shift((0,0,1))*scale(0.03,0.03,0.03)*unitsphere, opacity(0.9)+black,currentlight);

    surface s=surface(fs,(0,30),(72,60),10,5,Spline);
    draw(s,surfacepen=material(diffusepen=gray,emissivepen=black, specularpen=black));
    
    p=(75,-30);
    q=(75,60);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3);

    p=(81,60);
    q=(81,30);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3);

    p=(87,30);
    q=(87,120);
    draw(fs(p)..fs((p+q)/2)..fs(q),yarcPen,Arrow3);
    \end{asy}
    \caption{Caption}
    \label{fig:inversion}
\end{figure}
\subsubsection{Regular patches}

As shown in Fig.~\ref{fig:regular}, each regular patch corresponds to an axis-aligned rectangle in the parameter space, and each rectangle side is entirely shared by two adjacent patches.
In the context of such discretization, with the function value and its derivatives (i.e., $\bm{x}$, $\partial\bm{x}/\partial\xi^1$, $\partial\bm{x}/\partial\xi^2$, and $\partial^2\bm{x}/\partial\xi^1\partial\xi^2$) stored at nodes, 
the piecewise bicubic Hermite interpolation (\S\ref{apx:hermite}) can be used to naturally maintain the $\mathcal{C}^1$-smoothness and square-integrability (\S\ref{sec:theory_geometry}) in surface reconstruction.
 
It is easy to formulate the Hermite interpolation in an FEM-like style by converting the weights (\S\ref{apx:hermite}) into \emph{shape functions}.
Concretely speaking, the midsurface can be parameterized by 
\begin{equation}
  \label{eqn:shape}
  \bm{x}(\xi^1,\xi^2)=\sum_{I=1}^{N}\varPhi^I(\xi^1,\xi^2)\,\bm{q}_I\text{,}
\end{equation}
in which $\bm{q}_I\in\mathbb{R}^3$ ($I=1,2,3,\ldots,N$), treated as \emph{generalized coordinates}, denotes a value or derivative that is stored at nodes, and each $\bm{q}_I$ corresponds to a shape function $\varPhi^I(\xi^1,\xi^2)$.
These shape functions have compact supports, so the summand $\varPhi^I\bm{q}_I$ takes nonzero values only if $\bm{q}_I$ is stored at the $4$ nodes of the patch that $(\xi^1,\xi^2)$ lies in. Typically, the number of such $\bm{q}_I$ is $16$.

Regular patches can be readily used to discretize surfaces that are homeomorphic to a rectangle by embedding it in a Cartesian grid and taking grid cells as patches (Fig.~\ref{fig:regular}). More complex surfaces, e.g., cylinders and torus, can also be divided into regular patches with the help of periodic boundary conditions (\S\ref{sec:bhem_bc}), which is illustrated in Figs. \ref{fig:cylinder} and \ref{fig:torus}.

\subsubsection{Degenerate patches}

As demonstrated in Fig.~\ref{fig:degenerate}, sometimes singular points, surrounded by degenerate patches, are unavoidable in discretization.
A typical example is at the pole of a polar coordinate system (Fig.~\ref{fig:polar}), where the polar angle $\varphi$ takes arbitrary values such that one of the four edges collapses for each surrounding patch.
The $\mathcal{C}^1$-continuity there cannot be guaranteed by sharing first derivatives as usual, because there is no exact definition of the derivative w.r.t. the radius $r$ at a pole.

However, for a thin-shell geometry, it is not necessary to enforce $\mathcal{C}^1$-continuity everywhere.
As long as the midsurface is continuous and its normal vector exists at the poles, there are only discontinuities of first kind in the first- and second-order derivatives of $\bm{x}$, which does no harm to the integrability.
In other words, $\mathcal{G}^1$-continuity at poles and $\mathcal{C}^1$-continuity elsewhere is a sufficient condition for energy definition.
This suggests a straightforward workaround for degenerate patches.

Provided that there are two non-degenerate patches surrounding the pole $O$ in the parameter space, as illustrated in Fig.~\ref{fig:polar}, we respectively label the inner nodes as $A$, $B$, and $C$.
At each of these nodes, the radial coordinate $r$ is assumed to be a constant, denoted $\varepsilon_\mathrm{r}$, based on which the degenerate case can be analyzed by taking the limit as $\varepsilon_\mathrm{r}$ tends to zero.
To be specific, so as to enforce $\mathcal{G}^1$ around the pole, whatever the value of the polar coordinate $\varphi$ is, for any point of $\omega$ with zero-valued radial coordinate, the following conditions should be satisfied:
\begin{itemize}
  \item The function $\bm{x}(r,\varphi)$ takes the same value;
  \item The partial derivative $\partial\bm{x}/\partial r$ is coplanar.
\end{itemize}
According to properties of the Hermite interpolation, the former condition holds true within the given patches if and only if
\begin{subnumcases}{}
  \bm{x}_A=\bm{x}_B=\bm{x}_C\text{,}\\
  \frac{\partial\bm{x}}{\partial\varphi}\bigg|_A=\frac{\partial\bm{x}}{\partial\varphi}\bigg|_B=\frac{\partial\bm{x}}{\partial\varphi}\bigg|_C=\bm{0}\text{,}
\end{subnumcases}
while the latter can be met by establishing \emph{coplanar} generalized coordinates, which indicate that some $\bm{q}_I$ is a linear combination of two other regular generalized coordinates.
In the case of Fig.~\ref{fig:polar}, we can choose $\bm{e}_1=[\partial\bm{x}/\partial r]_A$ and $\bm{e}_2=[\partial\bm{x}/\partial r]_B$ as the basis, such that any coplanar vectors at the pole are represented by them. 

Below we investigate the radial derivative with $\varphi$ ranging from $\varphi_B$ to $\varphi_C$ as an example.
First, it is not hard to prove that all the derivatives stored at $B$ and $C$ must be in the plane formed by $\bm{e}_1$ and $\bm{e}_2$, which can be expanded as follows:
\begin{align}
[\partial\bm{x}/\partial r]_B&=m_B\bm{e}_1+n_B\bm{e}_2\text{,}\\
[\partial\bm{x}/\partial r]_C&=m_C\bm{e}_1+n_C\bm{e}_2\text{,}\\
[\partial^2\bm{x}/\partial\varphi\partial r]_B&=m'_B\bm{e}_1+n'_B\bm{e}_2\text{,}\\
[\partial^2\bm{x}/\partial\varphi\partial r]_C&=m'_C\bm{e}_1+n'_C\bm{e}_2\text{.}
\end{align}
Then, the radial derivative is interpolated by
{\footnotesize\begin{align}
\frac{\partial\bm{x}}{\partial r}(0,\varphi)={}&f(\theta)\frac{\partial\bm{x}}{\partial r}\bigg|_B+f(1-\theta)\frac{\partial\bm{x}}{\partial r}\bigg|_C+g(\theta)\frac{\partial^2\bm{x}}{\partial\varphi\partial r}\bigg|_B-g(1-\theta)\frac{\partial^2\bm{x}}{\partial\varphi\partial r}\bigg|_C\notag\\
={}&\left(f(\theta)m_B+f(1-\theta)m_C+g(\theta)m'_B-g(1-\theta)m'_C\right)\bm{e}_1\notag\\
&+\left(f(\theta)n_B+f(1-\theta)n_C+g(\theta)n'_B-g(1-\theta)n'_C\right)\bm{e}_2\text{,}\label{eqn:rad_drv}
\end{align}}%
in which the right-hand side can be abbreviated as $s_1(\theta)\,\bm{e}_1+s_2(\theta)\,\bm{e}_2$. Here, $\theta$ is calculated as $(\varphi-\varphi_B)/(\varphi_C-\varphi_B)$ ($\varphi_B\le\varphi\le\varphi_C$), and the functions $f$ and $g$ are used for the interpolation (\S\ref{apx:hermite}). Eq.~(\ref{eqn:rad_drv}) suggests that the interpolated radial derivative is also in the plane formed by $\bm{e}_1$ and $\bm{e}_2$, which is desired.
In addition, to ensure the existence of the unique normal vector at $O$, we must also restrict the orientation of the tangent plane when $\varphi$ takes different values, otherwise there may be inversion of $\bm{n}$, as shown in Fig.~\ref{fig:inversion}.
The additional condition can be formulated as
\begin{equation}
 \label{eqn:noninver}
 s(\theta)=s_1(\theta)\frac{\partial s_2}{\partial\theta}(\theta)-\frac{\partial s_1}{\partial\theta}(\theta)s_2(\theta)>0\text{,}
\end{equation}
whose proof is provided in \S\ref{apx:inversion}. 

In conclusion, when dealing with a singular point, we mark its surrounding patches as degenerate ones, whose inner nodes have the same positions and zero-valued polar coordinates that are enforced as boundary conditions (\S\ref{sec:bhem_bc}).
The other coordinates of these nodes, namely $\partial\bm{x}/\partial r$ and $\partial^2\bm{x}/\partial\varphi\partial r$, are treated as coplanar vectors, among which two vectors are chosen to be the basis and the others are constructed by linear combinations of them. The combination coefficients should further satisfy Eq.~(\ref{eqn:noninver}), which behaves like a penetration-free condition.
Given that there are $N_0$ regular vectors and $N_1$ degenerate vectors ($N=N_0+N_1$) among all the generalized coordinates, Eq.~(\ref{eqn:shape}) can be augmented with degenerate patches as
\begin{equation}
  \label{eqn:shape_plus}
  \bm{x}(\xi^1,\xi^2)=\sum_{I=1}^{N_0}\varPhi^I(\xi^1,\xi^2)\bm{q}_I
    +\sum_{R=1}^{2N_1}\varPsi^{R}(\xi^1,\xi^2)m_R\bm{q}_{i_R}\text{,}
\end{equation}
in which $m_R$ denotes a coefficient and $i_R$ ($1\le i_R\le N_0$) indicates an index of a regular vector. $\varPsi^R$ is a shape function derived from the Hermite interpolation, which is similar to $\varPhi^I$.


\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[trim=10cm 0cm 10cm 2.5cm,clip,width=0.163\textwidth]{#1}}
    \centering
    \formattedgraphics{Figures/can/patches_0119.0000.jpg}
    \formattedgraphics{Figures/can/patches_0119.0022.jpg}
    \formattedgraphics{Figures/can/patches_0119.0055.jpg}
    \formattedgraphics{Figures/can/patches_0119.0202.jpg}
    \formattedgraphics{Figures/can/patches_0119.0385.jpg}
        \formattedgraphics{Figures/can/patches_0119.0499.jpg}
    \caption{ A hollow cylindrical shell ($20\times20$ patches) deforms severely under the gradually increased compression. Initially, the cylinder is mounted on the ground; as the wood plank gets pushed down, the deformation of the cylinder manifests locally at first; at some point, the  unshaping takes a sudden change; further compression produces severe deformation and high degree of self contact.
}
    \label{fig:can}
    \vspace{-0.3cm}
\end{figure*}


\subsection{Boundary Conditions}
\label{sec:bhem_bc}


\paragraph*{Periodic boundary conditions.}
For BHEM simulations, it is significant to incorporate the periodic boundary conditions in order to complete geometric discretization.
As an example, in the discretization of a cylinder (Fig.~\ref{fig:cylinder}), a node with an azimuthal coordinate of $2\pi$ is identical to that with an azimuthal coordinate of $0$. Whenever we encounter such a situation, only one of the overlapping nodes need maintaining. Any calculation that involves these nodes is referred to the maintained one.

\paragraph*{Positional constraints.}
The BHEM prescribe two categories of positional constraints, namely Dirichlet and Neumann boundary conditions, which respectively constrain $\bm{x}(\xi^1,\xi^2)$ and its first-order derivatives at specific points.
When at nodes, these constraints can be simply realized by removing their corresponding generalized coordinates from the solution variables and taking their influence back to the governing equations as a given term.
Based on this, a constraint imposed on an elements' whole boundary curve can be realized through the combination of Dirichlet constraints and Neumann constraints along the boundary tangent direction for every node on the boundary.
Furthermore, as conventional finite element methods, Lagrange multipliers should be introduced to apply the constraints at arbitrary points of the midsurface.

\subsection{Governing Equations}

Now we consider discretizing Eq.~(\ref{eqn:dalembert1}) using the variational method based on the BH patches.
According to Eq.~(\ref{eqn:shape_plus}), the variation of $\bm{x}$ w.r.t. the DoFs are first calculated by 
\begin{equation}
  \label{eqn:delta_x}
  \delta\bm{x}=\sum_{I}\varPhi^I\delta\bm{q}_I
+\sum_{R}\varPsi^R(\delta m_R\,\bm{q}_{i_R}+m_R\,\delta\bm{q}_{i_R})\text{,}
\end{equation}
so we can define components of forces (w.r.t. the DoFs), denoted $\bm{F}_0^I$ and $F_1^R$, which satisfy
\begin{equation}
  \label{eqn:force_def}
  \iint_{\bar{\varOmega}}\bar{\bm{f}}\cdot\delta\bm{x}\,\mathrm{d}\bar{\varOmega}+\int_{\bar{\Gamma}}\bar{\bm{t}}\cdot\delta\bm{x}\,\mathrm{d}\bar{\Gamma}=\sum_I\bm{F}_0^I\cdot\delta\bm{q}_I+\sum_R F_1^R\delta m_R\text{.}
\end{equation}
And then $\delta T$ and $\delta V_\mathrm{e}$ are respectively investigated.

For the variation of the kinetic energy, the following equations are successively obtained by taking temporal derivatives:
\begin{gather}
  \dot{\bm{x}}=\sum_{J}\varPhi^J\dot{\bm{q}}_J
+\sum_{S}\varPsi^S(\dot{m}_S\bm{q}_{i_S}+m_S\dot{\bm{q}}_{i_S})\text{,}\\
  \ddot{\bm{x}}=\sum_{J}\varPhi^J\ddot{\bm{q}}_J
+\sum_{S}\varPsi^S(\ddot{m}_S\bm{q}_{i_S}+m_S\ddot{\bm{q}}_{i_S}+2\dot{m}_S\dot{\bm{q}}_{i_S})\text{.}
\end{gather}
Thus we can formulate $\delta T=\iint_{\bar{\varOmega}}\bar{\rho}h\ddot{\bm{x}}\cdot\delta\bm{x}\,\mathrm{d}\bar{\varOmega}$ as $\delta T_1+\delta T_2$:
\begin{align}
  \delta T_1&=\sum_{I}\left(\sum_{J}M_{00}^{IJ}\ddot{\bm{q}}_J+\sum_{S}\bm{M}_{01}^{IS}\ddot{m}_S-\hat{\bm{F}}_0^I\right)\cdot\delta\bm{q}_I\text{,}\label{eqn:delta_t1}\\
  \delta T_2&=\sum_{R}\left(\sum_{J}\bm{M}_{10}^{RJ}\cdot\ddot{\bm{q}}_J+\sum_{S}M_{11}^{RS}\ddot{m}_S-\hat{F}_1^R\right)\delta m_R\text{,}\label{eqn:delta_t2}
\end{align}
in which $M_{00}^{IJ}$, $\bm{M}_{01}^{IS}$, $\bm{M}_{10}^{RJ}$, and $M_{11}^{RS}$, as functions of $\{\bm{q}_I\}$ and $\{m_R\}$, are coefficients of mass matrices, while $\hat{\bm{F}}_0^I$ and $\hat{F}_1^R$, as functions of $\{\dot{\bm{q}}_I\}$ and $\{\dot{m}_R\}$, are components of fictitious forces.
Besides, for the variation of the elastic energy, since it does not directly depend on $\delta\bm{x}$, we need establish its expression with the help of partial derivatives as follows:
\begin{equation}
  \label{eqn:delta_ve}
  \delta V_\mathrm{e}=\iint_{\bar{\varOmega}}\left(\sum_{I}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\cdot\delta\bm{q}_I+\sum_{R}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial m_R}\delta m_R\right)\mathrm{d}\bar{\varOmega}\text{.}
\end{equation}
The detailed formulas of $\delta T$ and $\delta V_\mathrm{e}$ can be found in \S\ref{apx:variation}.

Substituting Eqs. (\ref{eqn:force_def}), (\ref{eqn:delta_t1}), (\ref{eqn:delta_t2}), and (\ref{eqn:delta_ve}), we reformulate Eq.~(\ref{eqn:dalembert1}) into a discretized version:
\begin{equation}
  \label{eqn:dalembert2}
  \sum_{I}\bm{\zeta}^I\cdot\delta\bm{q}_I+\sum_{R}\eta^{R}\delta m_{R}=0\text{,}
\end{equation}
in which coefficients $\bm{\zeta}_I$ and $\eta_{R}$ are calculated by
\begin{numcases}{}
\bm{\zeta}^I=\sum_{J}M_{00}^{IJ}\ddot{\bm{q}}_J+\sum_{S}\bm{M}_{01}^{IS}\ddot{m}_S+\iint_{\bar{\varOmega}}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial\bm{q}_I}\mathrm{d}\bar{\varOmega}-\hat{\bm{F}}_0^I-\bm{F}_0^I\text{,}\\
\eta^R=\sum_{J}\bm{M}_{10}^{RJ}\cdot\ddot{\bm{q}}_J+\sum_{S}M_{11}^{RS}\ddot{m}_S+\iint_{\bar{\varOmega}}\frac{\partial\bar{\mathcal{V}}_\mathrm{e}}{\partial m_R}\mathrm{d}\bar{\varOmega}-\hat{F}_1^R-F_1^R\text{.}
\end{numcases}
Since Eq.~(\ref{eqn:dalembert2}) holds for every possible variation, all of these coefficients must be equal to zero, i.e., $\bm{\zeta}^I=\bm{0}$ and $\eta^R=0$ for each $I$ and $R$, which govern the motion of a BHEM shell.
For static analysis, we only need to remove the contribution of $\delta T$ from the equations.


==> plot-backup.tex <==
\begin{figure}[ht]
  \centering
  \begin{tikzpicture}
    % \draw[step=0.4] (0,0) grid (2,2);
    % \fill (0,0) circle (0.05);
    % \fill (0,2) circle (0.05);
    % \fill (2,0) circle (0.05);
    % \fill (2,2) circle (0.05);
    % \node at(-0.2,-0.3) {$(0,0)$};
    % \node at(2.2,2.3) {$(1,1)$};
    % \node at(-0.2,2.3) {$(0,1)$};
    % \node at(2.2,-0.3) {$(1,0)$};
    % \draw[ultra thick,color={rgb,255:red,195; green,56; blue,40}] (1.2,0.8) rectangle (1.6,1.2);
    \draw (0,0) .. controls (2/3,0.5) and (4/3,-0.3) .. (2,0);
    \draw (2/9,2/3) .. controls (2/3,0.5) and (4/3,1) .. (20/9,2/3);
    \draw (4/9,4/3) .. controls (2/3,1) and (4/3,1.5) .. (22/9,4/3);
    \draw (2/3,2) .. controls (4/3,1.5) and (6/3,2.3) .. (8/3,2);
    \draw (0,0) -- (2/3,2);
    \draw (2,0) -- (8/3,2);
    % \draw[dashed,color={rgb,255:red,100; green,26; blue,17}] (1.4,0.8) -- (3.8,0.3);
    % \draw[dashed,color={rgb,255:red,100; green,26; blue,17}] (1.4,1.2) -- (3.8,1.7);
    %3.5-5.5,线头0.3
    % \draw[step=2] (4.3,0.3) grid (5.7,1.7);
    \draw (3.5,0.3) -- (5.5,0.3);
    \draw (3.5,1.7) -- (5.5,1.7);
    \draw (3.8,0) -- (3.8,2);
    \draw (5.2,0) -- (5.2,2);
    \fill (3.8,0.3) circle (0.05);
    \fill (3.8,1.7) circle (0.05);
    \fill (5.2,0.3) circle (0.05);
    \fill (5.2,1.7) circle (0.05);
    \node at(4.1,0.5) {$\bm{x}_{00}$};
    \node at(4.9,1.5) {$\bm{x}_{11}$};
    \node at(4.1,1.5) {$\bm{x}_{01}$};
    \node at(4.9,0.5) {$\bm{x}_{10}$};
    \node at(5.9,1.7) {$\xi_\mathrm{max}^2$};
    \node at(5.9,0.3) {$\xi_\mathrm{min}^2$};
    \node at(3.8,-0.3) {$\xi_\mathrm{min}^1$};
    \node at(5.2,-0.3) {$\xi_\mathrm{max}^1$};
    \node at(4.5,0.05) {$\Delta\xi^1$};
    \node[rotate=90] at(3.5,1) {$\Delta\xi^2$};
  \end{tikzpicture}
  \label{fig:regular}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.495\linewidth}
%     \begin{overpic}[width = \linewidth]{Figures/cylinder3.png}
%     \put(5,45){\small\color{red}{$u$}}
%     \put(35,10){\small\color{blue}{$v$}}
%     \end{overpic}
%     \caption{caption}
%     \end{subfigure}
%     \begin{subfigure}{0.495\linewidth}
%     \begin{overpic}[width = \linewidth]{Figures/torus1.png}
%     \put(20,35){\small\color{red}{$u$}}
%     \put(55,5){\small\color{blue}{$v$}}
%     \end{overpic}
%     \caption{caption}
%     \end{subfigure}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.495\linewidth}
    \centering
    \begin{tikzpicture}
    \def\R{1}
    \def\H{4}
    \def\angEl{-100}
    % \node[cylinder, draw, shape aspect=.5,minimum height=\H, minimum width=2*\R]{};
    \newcommand\Plane[3][current plane]{%
      \pgfmathsetmacro\xshift{\H * #3 / 160}
      \tikzset{#1/.style={cm={cos(\angEl),sin(\angEl)*sin(#2),0,cos(#2),(\xshift,0)}}} %
    }
    \newcommand\DrawCircle[2][1]{
      \Plane{0}{#2}
      \tikzset{current plane/.prefix style={scale=#1}}
      \draw[current plane,dashed] (90:1) arc (90:270:1);
      \draw[current plane] (90:1) arc (90:-90:1);
    }
    \newcommand\DrawLine[1]{
      \draw ({cos(-100)*\R*cos(#1)+\H/2},{\R*sin(#1)})--({cos(-100)*\R*cos(#1)-\H/2},{\R*sin(#1)});
    }
    \newcommand\DrawDashLine[1]{
      \draw[dashed] ({cos(-100)*\R*cos(#1)+\H/2},{\R*sin(#1)})--({cos(-100)*\R*cos(#1)-\H/2},{\R*sin(#1)});
    }
    % \shade [shading angle=90] (\H/2,0) arc (90:120:\R) -- +(-\H/2,0) arc (120:90:\R) -- cycle;
    \foreach \t in {-80,-60,...,80} { \DrawCircle[\R]{\t} }
    \foreach \t in {-80,-40,...,80} {\DrawLine{\t}}
    \foreach \t in {120,160,...,240} {\DrawDashLine{\t}}
    \DrawLine{90}
    \DrawLine{-90}
 %    \begin{axis}[
	% 	axis equal image,
	% 	hide axis,
	% 	z buffer = sort,
	% 	view = {122}{30},
	% 	scale = .7
	% ]
	% 	\addplot3[
	% 		surf,
	% 		shader = faceted interp,
	% 		samples = 10,
	% 		samples y = 20,
	% 		domain = 0:\H,
	% 		domain y = 0:2*pi,
	% 		colormap name = mycolormap,
	% 		thin,
	% 	](
	% 		{\R*sin(deg(\y))},
	% 		{\x},
	% 		{\R*cos(deg(\y))}
	% 	);
 %    \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \begin{subfigure}{0.495\linewidth}
    \centering
    \begin{tikzpicture}
    \def\R1{2}
 %    \begin{axis}[
	% 	axis equal image,
	% 	hide axis,
	% 	z buffer = sort,
	% 	view = {122}{30},
	% 	scale = .7
	% ]
	% 	\addplot3[
	% 		surf,
	% 		shader = faceted interp,
	% 		samples = 10,
	% 		samples y = 20,
	% 		domain = 0:2*pi,
	% 		domain y = 0:2*pi,
	% 		colormap name = mycolormap,
	% 		thin,
	% 	](
	% 		{(\R1+sin(deg(\x)))*cos(deg(\y))},
	% 		{(\R1+sin(deg(\x)))*sin(deg(\y))},
	% 		{cos(deg(\x))}
	% 	);
 %    \end{axis}
    \begin{axis}[colormap/blackwhite,
       view={30}{60},hide axis,scale = .7
       ]
       \addplot3[surf,shader=interp,
       samples=20,samples y=40,
       % patch type=biquadratic,
       point meta=x+3*z*z-0.25*y,
       domain=0:2*pi,y domain=0:2*pi,
       z buffer=sort]
       ({(1+0.5*cos(deg(x)))*cos(deg(y))}, 
        {(1+0.5*cos(deg(x)))*sin(deg(y))}, 
        {sin(deg(x))});
        \foreach \xx in {1,...,10}{
        \pgfmathsetmacro\xxx{\xx*2*pi/10}
        \addplot3+[domain=0:2*pi, line width=0.1mm, mark=none, color=black,samples y=10]
         ({(1+0.5*cos(deg(\xxx)))*cos(deg(x))}, 
        {(1+0.5*cos(deg(\xxx)))*sin(deg(x))}, 
        {sin(deg(\xxx))});
        }
        \foreach \yy in {1,...,10}{
        \pgfmathsetmacro\yyy{\yy*2*pi/10}
        \addplot3+[domain=0:2*pi, line width=0.1mm, mark=none, color=black,samples y=10]
         ({(1+0.5*cos(deg(x)))*cos(deg(\yyy))}, 
        {(1+0.5*cos(deg(x)))*sin(deg(\yyy))}, 
        {sin(deg(x))});
        }
   \end{axis}
    \end{tikzpicture}
    \end{subfigure}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\begin{tikzpicture}
%https://tex.stackexchange.com/questions/127238/how-do-you-draw-spheres-and-arcs-on-a-sphere-on-latex
\newcommand\pgfmathsinandcos[3]{%
  \pgfmathsetmacro#1{sin(#3)}%
  \pgfmathsetmacro#2{cos(#3)}%
}
\newcommand\LongitudePlane[3][current plane]{%
  \pgfmathsinandcos\sinEl\cosEl{#2} % elevation
  \pgfmathsinandcos\sint\cost{#3} % azimuth
  \tikzset{#1/.style={cm={\cost,\sint*\sinEl,0,\cosEl,(0,0)}}}
}
\newcommand\LatitudePlane[3][current plane]{%
  \pgfmathsinandcos\sinEl\cosEl{#2} % elevation
  \pgfmathsinandcos\sint\cost{#3} % latitude
  \pgfmathsetmacro\yshift{\cosEl*\sint}
  \tikzset{#1/.style={cm={\cost,0,0,\cost*\sinEl,(0,\yshift)}}} %
}
\newcommand\DrawLongitudeCircle[2][1]{
  \LongitudePlane{\angEl}{#2}
  \tikzset{current plane/.prefix style={scale=#1}}
   % angle of "visibility"
  \pgfmathsetmacro\angVis{atan(sin(#2)*cos(\angEl)/sin(\angEl))} %
  \draw[current plane] (\angVis:1) arc (\angVis:\angVis+180:1);
  \draw[current plane,dashed] (\angVis-180:1) arc (\angVis-180:\angVis:1);
  % \darw[current plane] (0,0) circle (1);
}
\newcommand\DrawLatitudeCircle[2][2]{
  \LatitudePlane{\angEl}{#2}
  \tikzset{current plane/.prefix style={scale=#1}}
  \pgfmathsetmacro\sinVis{sin(#2)/cos(#2)*sin(\angEl)/cos(\angEl)}
  % angle of "visibility"
  \pgfmathsetmacro\angVis{asin(min(1,max(\sinVis,-1)))}
  \draw[current plane] (\angVis:1) arc (\angVis:-\angVis-180:1);
  \draw[current plane,dashed] (180-\angVis:1) arc (180-\angVis:\angVis:1);
  % \darw[current plane] (0,0) circle (1);
}

\def\R{1.5} % sphere radius
\def\angEl{35} % elevation angle
\filldraw[ball color=white] (0,0) circle (\R);
\foreach \t in {-80,-60,...,80} { \DrawLatitudeCircle[\R]{\t} }
\foreach \t in {-5,-35,...,-175} { \DrawLongitudeCircle[\R]{\t} }
\end{tikzpicture}
